Snowmass Instrumentation Frontier IF02 Topical Group Report: Photon Detectors

The Photon Detectors Topical Group has identified two areas where focused R&D over the next decade could have a large impact in High Energy Physics Experiments. These areas described here are characterized by the convergence of a compelling scientific need and recent technological advances. Key messages: IF02-1 The development of detectors with the capability of counting single photons from IR to UV has been a very active area in the last decade. We now need to pursue R\&D to implement these in HEP experiments by making larger arrays, improving their energy resolution, timing, dark counts rates and extending their wavelength coverage. IF02-2 New photon detector developments are being considered for planned future neutrino experiments going beyond the current technologies. Concept demonstrations have been done, and we now need to move from a conceptual phase to working detectors. The science for generation, detection and manipulation of light is extremely fast moving and driven mainly from outside our field. The HEP community would benefit from resources dedicated to the implementation of these advanced photonic technologies in particle physics experiments.

==> Instrumentation/Header.tex <==


  \vfill

\begin{center}
\begin{Huge}   {\bf  TOPICAL GROUP REPORTS}

\bigskip

\bigskip

 {\bf Instrumentation  Frontier }

\vfill

\vfill

\end{Huge}
\end{center}

\newpage
\thispagestyle{empty}
\mbox{\null}




==> Instrumentation/IF02/bibliography.tex <==
\bibitem{Arapuca}
Machado A. A.,and Segreto E 
\newblock ARAPUCA a new device for liquid argon scintillation light detection.
\newblock{2016 JINST 11 C02004}
\bibitem{Vertical_drift}
Paulucci L. on behalf of the DUNE Collaboration
\newblock The DUNE vertical drift photon detection system.
\newblock{2022 JINST 17 C01067}
\bibitem{Young}
S. M. Young, M. Sarovar and F. Leonard
\newblock Nanoscale Architecture for Frequency-Resolving Single-Photon Detectors.
\newblock{arXiv:2205.05817v1}
\bibitem{Eftekharian}
A. Eftekharian, H. Atikian and A. Hamed Majedi
\newblock Plasmonic superconducting nanowire single photon detector.
\newblock{Optics Express Vol. 21, Issue 3, pp. 3043-3054 (2013) https://doi.org/10.1364/OE.21.003043 }
\bibitem{Miyata}
M. Miyata et al.
\newblock Full-color-sorting metalenses for high-sensitivity image sensors 
\newblock{Optica Vol. 8, Issue 12, pp. 1596-1604 (2021) •https://doi.org/10.1364/OPTICA.444255}
\bibitem{Klein}
Tanner Kaptanoglu, Meng Luo, Benjamin Land, Amanda Bacon, and Joshua R. Klein
\newblock Spectral photon sorting for large-scale Cherenkov and scintillation detectors.
\newblock{Phys. Rev. D 101, 072002 (2020)}
\bibitem{selenium}
S. K. Barman, M. N. Huda, J. Asaadi, E. Gramellini, D. Nygren
\newblock First principles studies of the surface and opto-electronic properties of ultra-thin t-Se.
\newblock{ arXiv:2104.14455v1}
\bibitem{organic}
M. Febbraro
\newblock Organic photosensors for detection of VUV scintillation light.
\newblock{Lidine 2021 this url: https://indico.physics.ucsd.edu/event/1/}
\bibitem{HyperK}
K. Abe et al.
\newblock Hyper-Kamiokande Design Report
\newblock{ arXiv:1805.04163v2}
\bibitem{Juno}
A. Abusleme et al
\newblock JUNO Physics and Detector.
\newblock{Progr. Part. Nucl. Phys.
123, (2022), 103927}
\bibitem{Dune}
DUNE Collaboration: B. Abi et al.
\newblock Long-baseline neutrino oscillation physics potential of the DUNE experiment.
\newblock{Eur. Phys. J. C 80, 978 (2020)}
\bibitem{Borexino}
M. Agostini et al. Borexino Coll.
\newblock First Directional Measurement of sub-MeV Solar Neutrinos with Borexino.
\newblock{https://doi.org/10.1103/PhysRevLett.128.091803
}
\bibitem{LAPPD}
 A. V. Lyashenko, B. W. Adams, M. Aviles, T. Cremer, C. D. Ertley, M. R. Foley, M. J. Minot, M. A. Popecki, M. E. Stochaj, W. A. Worstell, J. W. Elam, A. U. Mane, O. H. W. Siegmund, H. J. Frisch, A. L. Elagin, E. Angelico, E. Spieglan
 \newblock Performance of Large Area Picosecond Photo-Detectors (LAPPD).
 \newblock{https://doi.org/10.1016/j.nima.2019.162834}
 \bibitem{icarus}
  B. Ali-Mohammadzadeh, M. Babicz, W. Badgett, L. Bagby, V. Bellini, R. Benocci, M. Bonesini, A. Braggiotti, S. Centro, A. Chatterjee, A. G. Cocco, M. Diwan, A. Falcone, C. Farnese, A. Fava, D. Gibin, A. Guglielmi, W. Ketchum, U. Kose, A. Menegolli, G. Meng, C. Montanari, M. Nessi, F. Pietropaolo, A. Rappoldi , et al.
  \newblock Design and implementation of the new scintillation light detection system of ICARUS T600 
  \newblock{ 	
https://doi.org/10.48550/arXiv.2006.05261
Related DOI: 	
https://doi.org/10.1088/1748-0221/15/10/T10007}
\bibitem{SBND}
Abratenko, P. on behalf of the SBND Collaboration
\newblock Overview and Current Status of the X-ARAPUCA Light Collection System in SBND
\newblock{Lidine 2021 this url: https://indico.physics.ucsd.edu/event/1/contributions/42/}
\bibitem{I2-Scoresby}
J. Scoresby, ``Journals'', 1820.

\bibitem{I2-Beale}
A. Beale, ``Surgical Writings'', 1839.

\bibitem{GeCCD}
Digicam history.
\newblock
  \textsc{url:}~\url{http://www.digicamhistory.com/Evolutionary_Imagers.html}.

\bibitem{oscura_2020}
Oscura.
\newblock
  \textsc{url:}~\url{https://astro.fnal.gov/science/dark-matter/oscura/}, 2020.

\bibitem{Aalseth2021_DARKSIDE}
C.~E. Aalseth, S.~Abdelhakim, P.~Agnes, R.~Ajaj, I.~F.~M. Albuquerque,
  T.~Alexander, A.~Alici, A.~K. Alton, P.~Amaudruz, F.~Ameli, J.~Anstey,
  P.~Antonioli, M.~Arba, S.~Arcelli, R.~Ardito, I.~J. Arnquist, P.~Arpaia,
  D.~M. Asner, A.~Asunskis, M.~Ave, H.~O. Back, V.~Barbaryan,
  A.~Barrado~Olmedo, G.~Batignani, M.~G. Bisogni, V.~Bocci, A.~Bondar,
  G.~Bonfini, W.~Bonivento, E.~Borisova, B.~Bottino, M.~G. Boulay, R.~Bunker,
  S.~Bussino, A.~Buzulutskov, M.~Cadeddu, M.~Cadoni, A.~Caminata, N.~Canci,
  A.~Candela, C.~Cantini, M.~Caravati, M.~Cariello, F.~Carnesecchi,
  A.~Castellani, P.~Castello, P.~Cavalcante, D.~Cavazza, S.~Cavuoti,
  S.~Cebrian, J.~M. Cela~Ruiz, B.~Celano, R.~Cereseto, S.~Chashin, W.~Cheng,
  A.~Chepurnov, C.~Cical{\`o}, L.~Cifarelli, M.~Citterio, F.~Coccetti,
  V.~Cocco, M.~Colocci, E.~Conde~Vilda, L.~Consiglio, F.~Cossio, G.~Covone,
  P.~Crivelli, I.~D'Antone, M.~D'Incecco, M.~D. Da~Rocha~Rolo, O.~Dadoun,
  M.~Daniel, S.~Davini, S.~De~Cecco, M.~De~Deo, A.~De~Falco, D.~De~Gruttola,
  G.~De~Guido, G.~De~Rosa, G.~Dellacasa, P.~Demontis, S.~De~Pasquale, A.~V.
  Derbin, A.~Devoto, F.~Di Eusanio, L.~Di~Noto, G.~Di~Pietro, P.~Di~Stefano,
  C.~Dionisi, G.~Dolganov, F.~Dordei, M.~Downing, F.~Edalatfar, A.~Empl,
  M.~Fernandez~Diaz, C.~Filip, G.~Fiorillo, K.~Fomenko, A.~Franceschi,
  D.~Franco, E.~Frolov, G.~E. Froudakis, N.~Funicello, F.~Gabriele,
  A.~Gabrieli, C.~Galbiati, M.~Garbini, P.~Garcia~Abia,
  D.~Gasc{\~A}{\textthreesuperior}n~Fora, A.~Gendotti, C.~Ghiano, A.~Ghisi,
  P.~Giampa, R.~A. Giampaolo, C.~Giganti, M.~A. Giorgi, G.~K. Giovanetti, M.~L.
  Gligan, O.~Gorchakov, M.~Grab, R.~Graciani~Diaz, M.~Grassi, J.~W. Grate,
  A.~Grobov, M.~Gromov, M.~Guan, M.~B.~B. Guerra, M.~Guerzoni, M.~Gulino, R.~K.
  Haaland, B.~R. Hackett, A.~Hallin, M.~Haranczyk, B.~Harrop, E.~W. Hoppe,
  S.~Horikawa, B.~Hosseini, F.~Hubaut, P.~Humble, E.~V. Hungerford, An. Ianni,
  A.~Ilyasov, V.~Ippolito, C.~Jillings, K.~Keeter, C.~L. Kendziora,
  I.~Kochanek, K.~Kondo, G.~Kopp, D.~Korablev, G.~Korga, A.~Kubankin,
  R.~Kugathasan, M.~Kuss, M.~La~Commara, L.~La~Delfa, M.~Lai, M.~Lebois,
  B.~Lehnert, N.~Levashko, X.~Li, Q.~Liqiang, M.~Lissia, G.~U. Lodi, G.~Longo,
  R.~Lussana, L.~Luzzi, A.~A. Machado, I.~N. Machulin, A.~Mandarano,
  S.~Manecki, L.~Mapelli, A.~Margotti, S.~M. Mari, M.~Mariani, J.~Maricic,
  M.~Marinelli, D.~Marras, M.~Mart{\~A}­nez, A.~D. Martinez~Rojas, M.~Mascia,
  J.~Mason, A.~Masoni, A.~B. McDonald, A.~Messina, T.~Miletic, R.~Milincic,
  A.~Moggi, S.~Moioli, J.~Monroe, M.~Morrocchi, T.~Mroz, W.~Mu, V.~N. Muratova,
  S.~Murphy, C.~Muscas, P.~Musico, R.~Nania, T.~Napolitano, A.~Navrer~Agasson,
  M.~Nessi, I.~Nikulin, V.~Nosov, J.~A. Nowak, A.~Oleinik, V.~Oleynikov,
  M.~Orsini, F.~Ortica, L.~Pagani, M.~Pallavicini, S.~Palmas, L.~Pandola,
  E.~Pantic, E.~Paoloni, F.~Pazzona, S.~Peeters, P.~A. Pegoraro, K.~Pelczar,
  L.~A. Pellegrini, C.~Pellegrino, N.~Pelliccia, F.~Perotti, V.~Pesudo,
  E.~Picciau, F.~Pietropaolo, A.~Pocar, T.~R. Pollmann, D.~Portaluppi, S.~S.
  Poudel, P.~Pralavorio, D.~Price, B.~Radics, F.~Raffaelli, F.~Ragusa,
  M.~Razeti, C.~Regenfus, A.~L. Renshaw, S.~Rescia, M.~Rescigno, F.~Retiere,
  L.~P. Rignanese, C.~Ripoli, A.~Rivetti, J.~Rode, A.~Romani, L.~Romero,
  N.~Rossi, A.~Rubbia, P.~Sala, P.~Salatino, O.~Samoylov,
  E.~S{\~A}{\textexclamdown}nchez~Garc{\~A}­a, E.~Sandford, S.~Sanfilippo,
  M.~Sant, D.~Santone, R.~Santorelli, C.~Savarese, E.~Scapparone, B.~Schlitzer,
  G.~Scioli, E.~Segreto, A.~Seifert, D.~A. Semenov, A.~Shchagin, A.~Sheshukov,
  S.~Siddhanta, M.~Simeone, P.~N. Singh, P.~Skensved, M.~D. Skorokhvatov,
  O.~Smirnov, G.~Sobrero, A.~Sokolov, A.~Sotnikov, R.~Stainforth, A.~Steri,
  S.~Stracka, V.~Strickland, G.~B. Suffritti, S.~Sulis, Y.~Suvorov, A.~M.
  Szelc, R.~Tartaglia, G.~Testera, T.~Thorpe, A.~Tonazzo, A.~Tosi, M.~Tuveri,
  E.~V. Unzhakov, G.~Usai, A.~Vacca,
  E.~V{\~A}{\textexclamdown}zquez-J{\~A}{\textexclamdown}uregui, T.~Viant,
  S.~Viel, F.~Villa, A.~Vishneva, R.~B. Vogelaar, J.~Wahl, and J.~J. Walding.
\newblock Sipm-matrix readout of two-phase argon detectors using
  electroluminescence in the visible and near infrared range.
\newblock {\em The European Physical Journal C}, 81(2):153, Feb 2021.

\bibitem{article:MicroASe}
Shiva Abbaszadeh, I~Karim, and K~Vassili.
\newblock Measurement of uv from a microplasma by a microfabricated amorphous
  selenium detector.
\newblock {\em IEEE Transactions on Electron Devices}, 60:880--883, 02 2013.

\bibitem{Abdelhameed_20}
A.~H. Abdelhameed, P.~Angloher, G.~Bauer, et~al.
\newblock Deposition of tungsten thin films by magnetron sputtering for
  large-scale production of tungsten-based transition-edge sensors.
\newblock {\em J Low Temp Phys}, 199:401--407, 2020.

\bibitem{PhysRevLett.122.161801}
O.~Abramoff, L.~Barak, et~al.
\newblock Sensei: Direct-detection constraints on sub-gev dark matter from a
  shallow underground run using a prototype skipper ccd.
\newblock {\em Phys. Rev. Lett.}, 122:161801, Apr 2019.

\bibitem{sensei2019}
Orr Abramoff, Liron Barak, Itay~M. Bloch, Luke Chaplinsky, Michael Crisler,
  Dawa, Alex Drlica-Wagner, Rouven Essig, Juan Estrada, Erez Etzion, Guillermo
  Fernandez, Daniel Gift, Miguel Sofo-Haro, Joseph Taenzer, Javier Tiffenberg,
  Tomer Volansky, and Tien-Tien Yu.
\newblock Sensei: Direct-detection constraints on sub-gev dark matter from a
  shallow underground run using a prototype skipper ccd.
\newblock {\em Phys. Rev. Lett.}, 122:161801, Apr 2019.

\bibitem{acerbi2018silicon}
Fabio Acerbi, Giovanni Paternoster, Alberto Gola, Nicola Zorzi, and Claudio
  Piemonte.
\newblock Silicon photomultipliers and single-photon avalanche diodes with
  enhanced nir detection efficiency at fbk.
\newblock {\em Nuclear Instruments and Methods in Physics Research Section A:
  Accelerators, Spectrometers, Detectors and Associated Equipment},
  912:309--314, 2018.

\bibitem{AguilarPRL2017}
A.~Aguilar-Arevalo et~al.
\newblock First direct-detection constraints on ev-scale hidden-photon dark
  matter with {DAMIC} at {SNOLAB}.
\newblock {\em Physical Review Letters}, 118(14):141803, 2017.

\bibitem{cevns_2017}
D.~Akimov, J.~B. Albert, P.~An, C.~Awe, P.~S. Barbeau, B.~Becker, V.~Belov,
  A.~Brown, A.~Bolozdynya, B.~Cabrera-Palmer, M.~Cervantes, J.~I. Collar, R.~J.
  Cooper, R.~L. Cooper, C.~Cuesta, D.~J. Dean, J.~A. Detwiler, A.~Eberhardt,
  Y.~Efremenko, S.~R. Elliott, E.~M. Erkela, L.~Fabris, M.~Febbraro, N.~E.
  Fields, W.~Fox, Z.~Fu, A.~Galindo-Uribarri, M.~P. Green, M.~Hai, M.~R. Heath,
  S.~Hedges, D.~Hornback, T.~W. Hossbach, E.~B. Iverson, L.~J. Kaufman, S.~Ki,
  S.~R. Klein, A.~Khromov, A.~Konovalov, M.~Kremer, A.~Kumpan, C.~Leadbetter,
  L.~Li, W.~Lu, K.~Mann, D.~M. Markoff, K.~Miller, H.~Moreno, P.~E. Mueller,
  J.~Newby, J.~L. Orrell, C.~T. Overman, D.~S. Parno, S.~Penttila,
  G.~Perumpilly, H.~Ray, J.~Raybern, D.~Reyna, G.~C. Rich, D.~Rimal, D.~Rudik,
  K.~Scholberg, B.~J. Scholz, G.~Sinev, W.~M. Snow, V.~Sosnovtsev, A.~Shakirov,
  S.~Suchyta, B.~Suh, R.~Tayloe, R.~T. Thornton, I.~Tolstukhin, J.~Vanderwerp,
  R.~L. Varner, C.~J. Virtue, Z.~Wan, J.~Yoo, C.-H. Yu, A.~Zawada,
  J.~Zettlemoyer, A.~M. Zderic, and null null.
\newblock Observation of coherent elastic neutrino-nucleus scattering.
\newblock {\em Science}, 357(6356):1123--1126, 2017.

\bibitem{al2016backside}
T~Al~Abbas, NAW Dutton, O~Almer, S~Pellegrini, Y~Henrion, and RK~Henderson.
\newblock Backside illuminated spad image sensor with 7.83 $\mu$m pitch in
  3d-stacked cmos technology.
\newblock In {\em 2016 IEEE International Electron Devices Meeting (IEDM)},
  pages 8--1. IEEE, 2016.

\bibitem{allman2015near}
Michael~S Allman, Varun~B Verma, M~Stevens, Thomas Gerrits, Robert~D Horansky,
  Adriana~E Lita, Francesco Marsili, A~Beyer, MD~Shaw, D~Kumor, et~al.
\newblock A near-infrared 64-pixel superconducting nanowire single photon
  detector array with integrated multiplexed readout.
\newblock {\em Applied Physics Letters}, 106(19):192601, 2015.

\bibitem{Amare_05}
J.~Amar\'{e}, B.~Beltr\'{a}n, S.~Cebri\'{a}n, et~al.
\newblock Light yield of undoped sapphire at low temperature under particle
  excitation.
\newblock {\em APPLIED PHYSICS LETTERS}, 87:264102, 2005.

\bibitem{Ament-RMP-Ament}
Luuk J.~P. Ament, Michel van Veenendaal, Thomas~P. Devereaux, John~P. Hill, and
  Jeroen van~den Brink.
\newblock Resonant inelastic x-ray scattering studies of elementary
  excitations.
\newblock {\em Rev. Mod. Phys.}, 83:705--767, Jun 2011.

\bibitem{Angloher_16}
G.~Angloher, A.~Bento, C.~Bucci, et~al.
\newblock Results on light dark matter particles with a low-threshold
  {CRESST-II} detector.
\newblock {\em Eur. Phys. J. C}, 76:1--8, 2016.

\bibitem{1975-Cova_AQC-invention}
P.~Antognetti, S.~Cova, and A.~Longoni.
\newblock A study of the operation and performances of an avalanche diode as a
  single photon detector.
\newblock In {\em Proceedings of 2nd ispra nuclear electronics symp.}, {Stresa,
  Italy}, 1975.

\bibitem{apriledoke2006}
E.~Aprile, A.~E. Bolotnikov, A.~I. Bolozdynya, and T.~Doke.
\newblock {\em Noble Gas Detectors}.
\newblock John Wiley \& Sons, 2006.

\bibitem{ARPAIA201516}
R.~Arpaia, M.~Ejrnaes, L.~Parlato, F.~Tafuri, R.~Cristiano, D.~Golubev, Roman
  Sobolewski, T.~Bauch, F.~Lombardi, and G.P. Pepe.
\newblock High-temperature superconducting nanowires for photon detection.
\newblock {\em Physica C: Superconductivity and its Applications}, 509:16--21,
  2015.

\bibitem{Arvanitaki_18}
A.~Arvanitaki, S.~Dimopoulos, and K.~V. Tilburg.
\newblock Resonant absorption of bosonic dark matter in molecules.
\newblock {\em PHYSICAL REVIEW X}, 8:041001, 2018.

\bibitem{Asaadi:2018ixs}
J.~Asaadi, B.~J.~P. Jones, A.~Tripathi, I.~Parmaksiz, H.~Sullivan, and Z.~G.~R.
  Williams.
\newblock {Emanation and bulk fluorescence in liquid argon from tetraphenyl
  butadiene wavelength shifting coatings}.
\newblock {\em JINST}, 14(02):P02021, 2019.

\bibitem{1998-Aull_SPAD-3D}
BF~Aull, AH~Loomis, JA~Gregory, and DJ~Young.
\newblock Geiger-mode avalanche photodiode arrays integrated with {{CMOS}}
  timing circuits.
\newblock In {\em Device research conference digest, 1998. 56th annual}, pages
  58--59, {Charlottesville, USA,}, 1998. {IEEE}.

\bibitem{Aull2016}
Brian Aull.
\newblock Geiger-mode avalanche photodiode arrays integrated to all-digital
  {{CMOS}} circuits.
\newblock {\em Sensors}, 16(4), 2016.

\bibitem{aull2017large}
Brian~F Aull, Erik~K Duerr, Jonathan~P Frechette, K~Alexander McIntosh,
  Daniel~R Schuette, and Richard~D Younger.
\newblock Large-format geiger-mode avalanche photodiode arrays and readout
  circuits.
\newblock {\em IEEE Journal of Selected Topics in Quantum Electronics},
  24(2):1--10, 2017.

\bibitem{baba2018development}
Takashi Baba, Yoshihito Suzuki, Kenji Makino, Takuya Fujita, Tatsuya Hashi,
  Shunsuke Adachi, Shigeyuki Nakamura, and Koei Yamamoto.
\newblock Development of an ingaas spad 2d array for flash lidar.
\newblock In {\em Quantum Sensing and Nano Electronics and Photonics XV},
  volume 10540, page 105400L. International Society for Optics and Photonics,
  2018.

\bibitem{Barak:2020fql}
Liron Barak et~al.
\newblock {SENSEI: Direct-Detection Results on sub-GeV Dark Matter from a New
  Skipper-CCD}.
\newblock {\em Phys. Rev. Lett.}, 125(17):171802, 2020.

\bibitem{Baryakhtar_18}
M.~Baryakhtar, J.~Huang, and R.~Lasenby.
\newblock Axion and hidden photon dark matter detection with multilayer optical
  haloscopes.
\newblock {\em PHYSICAL REVIEW D}, 98:035006, 2018.

\bibitem{Baryakhtar2018}
Masha Baryakhtar, Junwu Huang, and Robert Lasenby.
\newblock Axion and hidden photon dark matter detection with multilayer optical
  haloscopes.
\newblock {\em Physical Review D}, 98(3):035006, 2018.

\bibitem{Bastidon_16}
N.~Bastidon, D.~Horns, A.~Lindner, et~al.
\newblock Quantum efficiency characterization and optimization of a tungsten
  {Transition-Edge Sensor} for {ALPS II}.
\newblock {\em J Low Temp Phys}, 184:88--90, 2016.

\bibitem{beer2018spad}
Maik Beer, Charles Thattil, Jan F~Haase, Jennifer Ruskowski, Werner Brockherde,
  and Rainer Kokozinski.
\newblock Spad-based lidar sensor in 0.35 $\mu$m automotive cmos with variable
  background light rejection.
\newblock In {\em Multidisciplinary Digital Publishing Institute Proceedings},
  volume 2(13), page 749, 2018.

\bibitem{Bender_20}
A.~N. Bender, A.~J. Anderson, J.~S. Avva, et~al.
\newblock On-sky performance of the {SPT-3G} frequency-domain multiplexed
  readout.
\newblock {\em J Low Temp. Phys.}, 199:182--191, 2020.

\bibitem{berchera2019quantum}
I~Ruo Berchera and Ivo~Pietro Degiovanni.
\newblock Quantum imaging with sub-poissonian light: challenges and
  perspectives in optical metrology.
\newblock {\em Metrologia}, 56(2):024001, 2019.

\bibitem{Bondaretal}
A.~Bondar, A.~Buzulutskov, A.~Dolgov, A.~Grebenuk, E.~Shemyakina, and
  A.~Sokolov.
\newblock Study of infrared scintillations in gaseous and liquid argon - part
  i: methodology and time measurements.
\newblock {\em JINST}, 7:06015, 2012.

\bibitem{Borghesanijchemphys}
A.~F. Borghesani, G.~Bressi, G.~Carugno, E.~Conti, and D.~Ianuzzi.
\newblock Infrared fluorescence of xe2 molecules in electron/proton beam
  excited pure xe gas and in an ar/xe gas mixture.
\newblock {\em J. Chem. Phys.}, 115:6042, 2001.

\bibitem{boulenc2017high}
Pierre Boulenc, Jo~Robbelein, Linkun Wu, Luc Haspeslagh, Piet De~Moor, Jonathan
  Borremans, and Maarten Rosmeulen.
\newblock High speed tdi embedded ccd in cmos sensor.
\newblock In {\em International Conference on Space Optics—ICSO 2016}, volume
  10562, page 105622P. International Society for Optics and Photonics, 2017.

\bibitem{bressiPLA}
G.~Bressi, G.~Carugno, E.~Conti, D.~Ianuzzi, and A.~T. Meneguzzo.
\newblock A first study of the infrared emission in argon excited by ionizing
  particles.
\newblock {\em Phys. Lett.}, A278:280--285, 2001.

\bibitem{Brida:10}
Giorgio Brida, Ivo~Pietro Degiovanni, Marco Genovese, Maria~Luisa Rastello, and
  Ivano Ruo-Berchera.
\newblock Detection of multimode spatial correlation in pdc and application to
  the absolute calibration of a ccd camera.
\newblock {\em Opt. Express}, 18(20):20572--20584, Sep 2010.

\bibitem{brida2010experimental}
Giorgio Brida, Marco Genovese, and I~Ruo Berchera.
\newblock Experimental realization of sub-shot-noise quantum imaging.
\newblock {\em Nature Photonics}, 4(4):227--230, 2010.

\bibitem{bruschini2019single}
Claudio Bruschini, Harald Homulle, Ivan~Michel Antolovic, Samuel Burri, and
  Edoardo Charbon.
\newblock Single-photon avalanche diode imagers in biophotonics: review and
  outlook.
\newblock {\em Light: Science \& Applications}, 8(1):1--28, 2019.

\bibitem{Burney_06}
J.~Burneya, T.~J. Baya, J.~Barral, et~al.
\newblock Transition-edge sensor arrays for {UV-optical-IR} astrophysics.
\newblock {\em Nuclear Instruments and Methods in Physics Research A},
  559:525–527, 2006.

\bibitem{Cabreraa_00}
B.~Cabrera, R.~Clarke, A.~Milleret, et~al.
\newblock Cryogenic detectors based on superconducting transition-edge sensors
  for time-energy-resolved single-photon counters and for dark matter searches.
\newblock {\em Physica B}, 280:509--514, 2000.

\bibitem{cahall2017multi}
Clinton Cahall, Kathryn~L Nicolich, Nurul~T Islam, Gregory~P Lafyatis, Aaron~J
  Miller, Daniel~J Gauthier, and Jungsang Kim.
\newblock Multi-photon detection using a conventional superconducting nanowire
  single-photon detector.
\newblock {\em Optica}, 4(12):1534--1535, 2017.

\bibitem{Caldwell_17}
A.~Caldwell, B.~Dvali, G.~Majorovits, et~al.
\newblock {Dielectric Haloscopes: A New Way to Detect Axion Dark Matter}.
\newblock {\em Phys. Rev. Lett.}, 118:0091801, 2017.

\bibitem{inproceedings:aSeCMOS}
A.~Camlica, A.~El-Falou, R.~Mohammadi, P.~Levine, and K.~Karim.
\newblock Cmos-integrated single-photon-counting x-ray detector using an
  amorphous-selenium photoconductor with $11\times 11-\mu \mathbf{m}^{2}$
  pixels.
\newblock In {\em 2018 IEEE International Electron Devices Meeting (IEDM)},
  pages 32.5.1--32.5.4, 12 2018.

\bibitem{lta_2021}
Gustavo {Cancelo}, Claudio {Chavez}, Fernando {Chierchie}, Juan {Estrada},
  Guillermo~Fernandez {Moroni}, Eduardo {Paolini}, Miguel~Sofo {Haro}, Angel
  {Soto}, Leandro {Stefanazzi}, Javier {Tiffenberg}, Ken {Treptow}, Neal
  {Wilcer}, and Ted {Zmuda}.
\newblock {Low threshold acquisition controller for Skipper charge-coupled
  devices}.
\newblock {\em Journal of Astronomical Telescopes, Instruments, and Systems},
  7:015001, January 2021.

\bibitem{Cao2018}
Yuan Cao, Valla Fatemi, Shiang Fang, Kenji Watanabe, Takashi Taniguchi,
  Efthimios Kaxiras, and Pablo Jarillo-Herrero.
\newblock Unconventional superconductivity in magic-angle graphene
  superlattices.
\newblock {\em Nature}, 556(7699):43--50, Apr 2018.

\bibitem{Carr-prb}
Stephen Carr, Daniel Massatt, Shiang Fang, Paul Cazeaux, Mitchell Luskin, and
  Efthimios Kaxiras.
\newblock Twistronics: Manipulating the electronic properties of
  two-dimensional layered structures through their twist angle.
\newblock {\em Phys. Rev. B}, 95:075420, Feb 2017.

\bibitem{Carter_17}
F.~W. Carter, S.~A. Hertel, M.~J. Rooks, et~al.
\newblock Calorimetric observation of single {He$_2^*$} excimers in a {100-mK
  He} bath.
\newblock {\em J Low Temp Phys}, 186:183--196, 2017.

\bibitem{DMfacilitiesWP}
Sukanya Chakrabarti et~al.
\newblock {Snowmass2021 Cosmic Frontier White Paper: Observational Facilities
  to Study Dark Matter}.
\newblock In {\em Contribution to Snowmass 2021}, 2022.

\bibitem{Chen2008}
Hsiang-Yu Chen, Michael K.~F. Lo, Guanwen Yang, Harold~G. Monbouquette, and
  Yang Yang.
\newblock Nanoparticle-assisted high photoconductive gain in composites of
  polymer and fullerene.
\newblock {\em Nature Nanotechnology}, 3(9):543--547, 2008.

\bibitem{Cherednichenko_2021}
Sergey Cherednichenko, Narendra Acharya, Evgenii Novoselov, and Vladimir
  Drakinskiy.
\newblock Low kinetic inductance superconducting {MgB}2 nanowires with a 130 ps
  relaxation time for single-photon detection applications.
\newblock {\em Superconductor Science and Technology}, 34(4):044001, feb 2021.

\bibitem{smart_skipper_2021}
Fernando Chierchie, Guillermo~Fernandez Moroni, Leandro Stefanazzi, Eduardo
  Paolini, Javier Tiffenberg, Juan Estrada, Gustavo Cancelo, and Sho Uemura.
\newblock Smart readout of nondestructive image sensors with single
  photon-electron sensitivity.
\newblock {\em Phys. Rev. Lett.}, 127:241101, Dec 2021.

\bibitem{Chiles:2021}
Jeff Chiles, Ilya Charaev, Robert Lasenby, Masha Baryakhtar, Junwu Huang,
  Alexana Roshko, George Burton, Marco Colangelo, Ken Van~Tilburg, Asimina
  Arvanitaki, Sae-Woo Nam, and Karl Berggren.
\newblock First constraints on dark photon dark matter with superconducting
  nanowire detectors in an optical haloscope.
\newblock {\em arXiv preprint arXiv:2110.01582}, 10 2021.

\bibitem{Coropceanu2007}
Veaceslav Coropceanu, Jérôme Cornil, Demetrio~A. da~Silva~Filho, Yoann
  Olivier, Robert Silbey, and Jean-Luc Brédas.
\newblock Charge transport in organic semiconductors.
\newblock {\em Chemical Reviews}, 107(4):926--952, 2007.
\newblock PMID: 17378615.

\bibitem{hamamatsu_technote}
Hamamatsu Corporation.
\newblock Orca-quest qcmos camera, technical note.
\newblock
  \textsc{url:}~\url{https://www.hamamatsu.com/content/dam/hamamatsu-photonics/sites/documents/99_SALES_LIBRARY/sys/SCAS0154E_C15550-20UP_tec.pdf}{Hamamatsu.com},
  September 2021.

\bibitem{hamamatsu_whitepaper}
Hamamatsu Corporation.
\newblock qcmos: Quantitative cmos technology enabled by photon number
  resolving, white paper.
\newblock
  \textsc{url:}~\url{https://www.hamamatsu.com/content/dam/hamamatsu-photonics/sites/documents/99_SALES_LIBRARY/sys/SCAS0149E_qCMOS_whitepaper.pdf},
  April 2021.

\bibitem{hamamatsu_nirenhancedsipm}
Hamamatsu Corporation.
\newblock Near infrared high sensitivity mppc: S15639-1325ps.
\newblock
  \textsc{url:}~\url{https://www.hamamatsu.com/us/en/product/optical-sensors/mppc/mppc_mppc-array.html},
  March 2022.

\bibitem{cova1996avalanche}
Sergio Cova, Massimo Ghioni, Andrea Lacaita, Carlo Samori, and Franco Zappa.
\newblock Avalanche photodiodes and quenching circuits for single-photon
  detection.
\newblock {\em Applied optics}, 35(12):1956--1976, 1996.

\bibitem{sensei2018}
Michael {Crisler}, Rouven {Essig}, Juan {Estrada}, Guillermo {Fernand ez},
  Javier {Tiffenberg}, Miguel~Sofo {Haro}, Tomer {Volansky}, Tien-Tien {Yu},
  and {Sensei Collaboration}.
\newblock {SENSEI: First Direct-Detection Constraints on Sub-GeV Dark Matter
  from a Surface Run}.
\newblock {\em \textit{PRL}}, 121(6):061803, Aug 2018.

\bibitem{crooks2013kirana}
J~Crooks, B~Marsh, R~Turchetta, K~Taylor, W~Chan, A~Lahav, and Amos Fenigstein.
\newblock Kirana: a solid-state megapixel ucmos image sensor for ultrahigh
  speed imaging.
\newblock In {\em Sensors, cameras, and systems for industrial and scientific
  applications XIV}, volume 8659, page 865903. International Society for Optics
  and Photonics, 2013.

\bibitem{1993-Dautet-McIntyre_Photon-Counting}
H.~Dautet, P.~Deschamps, B.~Dion, A.~D. MacGregor, D.~MacSween, R.~J. McIntyre,
  C.~Trottier, and P.~P. Webb.
\newblock Photon counting techniques with silicon avalanche photodiodes.
\newblock {\em Applied Optics}, 32(21):3894--3900, 1993.

\bibitem{dautet1993photon}
Henri Dautet, Pierre Deschamps, Bruno Dion, Andrew~D MacGregor, Darleene
  MacSween, Robert~J McIntyre, Claude Trottier, and Paul~P Webb.
\newblock Photon counting techniques with silicon avalanche photodiodes.
\newblock {\em Applied optics}, 32(21):3894--3900, 1993.

\bibitem{2018arXiv180207216D}
Kyle {Dawson}, Josh {Frieman}, Katrin {Heitmann}, Bhuvnesh {Jain}, Steve
  {Kahn}, Rachel {Mandelbaum}, Saul {Perlmutter}, and An{\v{z}}e {Slosar}.
\newblock {Cosmic Visions Dark Energy: Small Projects Portfolio}.
\newblock {\em arXiv e-prints}, page arXiv:1802.07216, Feb 2018.

\bibitem{dawson2019maintaining}
Kyle Dawson, Stephen Holland, and David Schlegel.
\newblock Maintaining capabilities in ccd production for the astronomy
  community.
\newblock {\em arXiv preprint arXiv:1907.06798}, 2019.

\bibitem{2003Natur.425..817D}
Peter~K Day, Henry~G Leduc, Benjamin~A Mazin, Anastasios Vayonakis, and Jonas
  Zmuidzinas.
\newblock {A broadband superconducting detector suitable for use in large
  arrays}.
\newblock {\em Nature}, 425(6):817--821, October 2003.

\bibitem{Derenzo_17}
S.~Derenzo, R.~Essig, A.~Massari, et~al.
\newblock Direct detection of {sub-GeV} dark matter with scintillating targets.
\newblock {\em Phys. Rev. D}, 96:016126, 2017.

\bibitem{PhysRevD.96.016026}
Stephen Derenzo, Rouven Essig, Andrea Massari, Adri\'an Soto, and Tien-Tien Yu.
\newblock Direct detection of sub-gev dark matter with scintillating targets.
\newblock {\em Phys. Rev. D}, 96:016026, Jul 2017.

\bibitem{mpd_pdmir}
Micro~Photon Devices.
\newblock Pdm-ir.
\newblock
  \textsc{url:}~\url{http://www.micro-photon-devices.com/MPD/media/Datasheet/PDM-IR\%20Datasheet\%20window.pdf},
  March 2022.

\bibitem{Dober_21}
B.~Dober, Z.~Ahmed, K.~Arnold, et~al.
\newblock A microwave {SQUID} multiplexer optimized for bolometric
  applications.
\newblock {\em Appl. Phys. Lett.}, 118:062601, 2021.

\bibitem{donnelly2006design}
Joseph~P Donnelly, Erik~K Duerr, K~Alex McIntosh, Eric~A Dauler, Douglas~C
  Oakley, Steven~H Groves, Christopher~J Vineis, Leonard~J Mahoney, Karen~M
  Molvar, Pablo~I Hopman, et~al.
\newblock Design considerations for 1.06-$ mu $ m ingaasp--inp geiger-mode
  avalanche photodiodes.
\newblock {\em IEEE Journal of Quantum Electronics}, 42(8):797--809, 2006.

\bibitem{Doriesel_16}
W.~B. Doriese1, K.~M. Morgan1, D.~A. Bennett, et~al.
\newblock Developments in {Time-Division Multiplexing of X-ray Transition-Edge
  Sensors}.
\newblock {\em J Low Temp. Phys.}, 184:389--195, 2016.

\bibitem{Eschweiler_15}
J.~Dreyling-Eschweiler, N.~Bastidon, B.~D\"{o}brich, et~al.
\newblock “characterization, 1064 nm photon signals and background events of
  a tungsten {TES} detector for the {ALPS} experiment.
\newblock {\em Journal of Modern Optics}, 62:1132--1140, 2015.

\bibitem{Drlica-Wagner:2020}
Alex {Drlica-Wagner}, Edgar {Marrufo Villalpando}, Judah {O'Neil}, Juan
  {Estrada}, Stephen {Holland}, Noah {Kurinsky}, Ting {Li}, Guillermo
  {Fernandez Moroni}, Javier {Tiffenberg}, and Sho {Uemura}.
\newblock {Characterization of skipper CCDs for cosmological applications}.
\newblock In {\em Society of Photo-Optical Instrumentation Engineers (SPIE)
  Conference Series}, volume 11454 of {\em Society of Photo-Optical
  Instrumentation Engineers (SPIE) Conference Series}, page 114541A, December
  2020.

\bibitem{Erdal:2016jhl}
E.~Erdal, L.~Arazi, M.~L. Rappaport, S.~Shchemelinin, D.~Vartsky, and
  A.~Breskin.
\newblock {First demonstration of VUV-photon detection in liquid xenon with
  THGEM and GEM-based Liquid Hole Multipliers}.
\newblock {\em Nucl. Instrum. Meth.}, A845:218--221, 2017.

\bibitem{Essig_19}
R.~Essig, J.~P\'{e}rez-Ríos, H.~Ramani, and O.~Slone.
\newblock Direct detection of nuclear scattering of {sub-GeV} dark matter using
  molecular excitation.
\newblock {\em Phys. Rev. Research}, 1:033105, 2019.

\bibitem{fernandez2021LightMediators}
G~Fernandez-Moroni, R~Harnik, PAN Machado, I~Martinez-Soler, YF~Perez-Gonzalez,
  D~Rodrigues, and S~Rosauro-Alcaraz.
\newblock The physics potential of a reactor neutrino experiment with
  skipper-ccds: Searching for new physics with light mediators.
\newblock {\em arXiv preprint arXiv:2108.07310}, 2021.

\bibitem{skipper_2012}
Guillermo Fernandez~Moroni, Juan Estrada, G.~Cancelo, Stephen Holland, Eduardo
  Paolini, and H.~Diehl.
\newblock Sub-electron readout noise in a skipper ccd fabricated on high
  resistivity silicon.
\newblock {\em Experimental Astronomy}, 34, 07 2012.

\bibitem{fernandez2021WeakMixing}
Guillermo Fernandez-Moroni, Pedro~AN Machado, Ivan Martinez-Soler, Yuber~F
  Perez-Gonzalez, Dario Rodrigues, and Salvador Rosauro-Alcaraz.
\newblock The physics potential of a reactor neutrino experiment with skipper
  ccds: Measuring the weak mixing angle.
\newblock {\em Journal of High Energy Physics}, 2021(3):1--25, 2021.

\bibitem{Ferrari2016}
Eugenio Ferrari, Carlo Spezzani, Franck Fortuna, Renaud Delaunay, Franck Vidal,
  Ivaylo Nikolov, Paolo Cinquegrana, Bruno Diviacco, David Gauthier, Giuseppe
  Penco, Primo{\v{z}}~Rebernik Ribi{\v{c}}, Eleonore Roussel, Marco Trov{\`o},
  Jean-Baptiste Moussy, Tommaso Pincelli, Loun{\`e}s Lounis, Michele Manfredda,
  Emanuele Pedersoli, Flavio Capotondi, Cristian Svetina, Nicola Mahne, Marco
  Zangrando, Lorenzo Raimondi, Alexander Demidovich, Luca Giannessi, Giovanni
  De~Ninno, Miltcho~Boyanov Danailov, Enrico Allaria, and Maurizio Sacchi.
\newblock Widely tunable two-colour seeded free-electron laser source for
  resonant-pump resonant-probe magnetic scattering.
\newblock {\em Nature Communications}, 7(1):10343, Jan 2016.

\bibitem{Fert2017}
Albert Fert, Nicolas Reyren, and Vincent Cros.
\newblock Magnetic skyrmions: advances in physics and potential applications.
\newblock {\em Nature Reviews Materials}, 2(7):17031, Jun 2017.

\bibitem{fife2009design}
Keith Fife, Abbas El~Gamal, and H-S~Philip Wong.
\newblock Design and characterization of submicron ccds in cmos.
\newblock In {\em International Image Sensor Workshop}, 2009.

\bibitem{Fink_20}
C.~W. Fink, S.~L. Watkins, T.~Aramaki, et~al.
\newblock Characterizing {TES} power noise for future single optical-phonon and
  infrared-photon detectors.
\newblock {\em AIP Advances}, 10:085221, 2020.

\bibitem{QIS_whitepaper}
Eric Fossum, Jiaju Ma, Saleh Masoodian, Leo Anzagira, and Rachel Zizza.
\newblock The quanta image sensor: Every photon counts.
\newblock
  \textsc{url:}~\url{https://digitalcommons.dartmouth.edu/cgi/viewcontent.cgi?article=4432&context=facoa},
  October 2016.

\bibitem{fossum2014review}
Eric~R Fossum and Donald~B Hondongwa.
\newblock A review of the pinned photodiode for ccd and cmos image sensors.
\newblock {\em IEEE Journal of the electron devices society}, 2014.

\bibitem{fowler20105}
Boyd Fowler, Chiao Liu, Steve Mims, Janusz Balicki, Wang Li, Hung Do, Jeff
  Appelbaum, and Paul Vu.
\newblock A 5.5 mpixel 100 frames/sec wide dynamic range low noise cmos image
  sensor for scientific applications.
\newblock In {\em Sensors, Cameras, and Systems for Industrial/Scientific
  Applications XI}, volume 7536, page 753607. International Society for Optics
  and Photonics, 2010.

\bibitem{FreedmanCEVENS1974}
Daniel~Z. Freedman.
\newblock Coherent effects of a weak neutral current.
\newblock {\em Phys. Rev. D}, 9:1389--1392, Mar 1974.

\bibitem{Fuentes-Hernandez2020}
Canek Fuentes-Hernandez, Wen-Fang Chou, Talha~M. Khan, Larissa Diniz, Julia
  Lukens, Felipe~A. Larrain, Victor~A. Rodriguez-Toro, and Bernard Kippelen.
\newblock Large-area low-noise flexible organic photodiodes for detecting faint
  visible light.
\newblock {\em Science}, 370(6517):698--701, 2020.

\bibitem{Fujino_11}
H.~Fujino, H.~Ishii, T.~Itatani, et~al.
\newblock Titanium-based transition-edge photon number resolving detector with
  98\% detection efficiency with index-matched small-gap fiber coupling.
\newblock {\em Opt. Express}, 19:870--875, 2011.

\bibitem{Fukuda_09}
D.~Fukuda, G.~Fujii, T.~Numata, et~al.
\newblock Photon number resolving detection with high speed and high quantum
  efficiency.
\newblock {\em Metrologia}, 46:S288, 2009.

\bibitem{gallina2019characterization}
G.~Gallina, P.~Giampa, F.~RetiÃšre, J.~Kroeger, G.~Zhang, M.~Ward,
  P.~Margetak, G.~Li, T.~Tsang, L.~Doria, S.~{Al Kharusi}, M.~Alfaris,
  G.~Anton, I.J. Arnquist, I.~Badhrees, P.S. Barbeau, D.~Beck, V.~Belov,
  T.~Bhatta, J.~Blatchford, J.P. Brodsky, E.~Brown, T.~Brunner, G.F. Cao,
  L.~Cao, W.R. Cen, C.~Chambers, S.A. Charlebois, M.~Chiu, B.~Cleveland,
  M.~Coon, A.~Craycraft, J.~Dalmasson, T.~Daniels, L.~Darroch, S.J. Daugherty,
  A.~{De St. Croix}, A.~{Der Mesrobian-Kabakian}, R.~DeVoe, J.~Dilling, Y.Y.
  Ding, M.J. Dolinski, A.~Dragone, J.~Echevers, M.~Elbeltagi, L.~Fabris,
  D.~Fairbank, W.~Fairbank, J.~Farine, S.~Feyzbakhsh, R.~Fontaine, P.~Gautam,
  G.~Giacomini, R.~Gornea, G.~Gratta, E.V. Hansen, M.~Heffner, E.W. Hoppe,
  J.~H{\"o}{\ss}l, A.~House, M.~Hughes, Y.~Ito, A.~Iverson, A.~Jamil, M.J.
  Jewell, X.S. Jiang, A.~Karelin, L.J. Kaufman, D.~Kodroff, T.~Koffas,
  R.~Krücken, A.~Kuchenkov, K.S. Kumar, Y.~Lan, A.~Larson, B.G. Lenardo, D.S.
  Leonard, S.~Li, Z.~Li, C.~Licciardi, Y.H. Lin, P.~Lv, R.~MacLellan,
  T.~McElroy, M.~Medina-Peregrina, T.~Michel, B.~Mong, D.C. Moore, K.~Murray,
  P.~Nakarmi, R.J. Newby, Z.~Ning, O.~Njoya, F.~Nolet, O.~Nusair, K.~Odgers,
  A.~Odian, M.~Oriunno, J.L. Orrell, G.S. Ortega, I.~Ostrovskiy, C.T. Overman,
  S.~Parent, A.~Piepke, A.~Pocar, J.-F. Pratte, D.~Qiu, V.~Radeka, E.~Raguzin,
  S.~Rescia, M.~Richman, A.~Robinson, T.~Rossignol, P.C. Rowson, N.~Roy,
  R.~Saldanha, S.~Sangiorgio, K.~Skarpaas, A.K. Soma, G.~St-Hilaire,
  V.~Stekhanov, T.~Stiegler, X.L. Sun, M.~Tarka, J.~Todd, T.~Tolba, T.I. Totev,
  R.~Tsang, F.~Vachon, V.~Veeraraghavan, G.~Visser, J.-L. Vuilleumier,
  M.~Wagenpfeil, M.~Walent, Q.~Wang, J.~Watkins, M.~Weber, W.~Wei, L.J. Wen,
  U.~Wichoski, S.X. Wu, W.H. Wu, X.~Wu, Q.~Xia, H.~Yang, L.~Yang, Y.-R. Yen,
  O.~Zeldovich, J.~Zhao, Y.~Zhou, and T.~Ziegler.
\newblock Characterization of the hamamatsu vuv4 mppcs for nexo.
\newblock {\em Nuclear Instruments and Methods in Physics Research Section A:
  Accelerators, Spectrometers, Detectors and Associated Equipment},
  940:371--379, 2019.

\bibitem{Giazotto_06}
F.~Giazotto, T.~T. Heikkil\"{a}, A.~Luukanen, et~al.
\newblock Opportunities for mesoscopics in thermometry and refrigeration:
  Physics and applications.
\newblock {\em Rev. Mod. Phys.}, 78:217, 2006.

\bibitem{giovanetti2011}
V~Giovannetti, S~Lloyd, and L~Maccone.
\newblock Advances in quantum metrology.
\newblock {\em Nature Photonics}, 5(4):222–229, 2011.

\bibitem{Goodenough2010}
John~B. Goodenough and Youngsik Kim.
\newblock Challenges for rechargeable li batteries.
\newblock {\em Chemistry of Materials}, 22(3):587--603, Feb 2010.

\bibitem{gulinatti2012new}
Angelo Gulinatti, Ivan Rech, Francesco Panzeri, Corrado Cammi, P~Maccagnani,
  M~Ghioni, and Sergio Cova.
\newblock New silicon spad technology for enhanced red-sensitivity,
  high-resolution timing and system integration.
\newblock {\em Journal of Modern Optics}, 59(17):1489--1499, 2012.

\bibitem{hadfield2009single}
Robert~H Hadfield.
\newblock Single-photon detectors for optical quantum information applications.
\newblock {\em Nature photonics}, 3(12):696--705, 2009.

\bibitem{he-2021-natphys}
M.~He, Y.~Li, J.~Cai, Y.~Liu, K.~Watanabe, X.~Xu, and M.~Yankowitz.
\newblock Symmetry breaking in twisted double bilayer graphene.
\newblock {\em Nature Physics}, 17:26--30, 2020.

\bibitem{HeindlJINST}
T.~Heindl, T.~Dandl, M.~Hofmann, R.~Krücken, L.~Oberauer, W.~Potzel,
  J.~Wieser, and A.~Ulrich.
\newblock The scintillation of liquid argon.
\newblock {\em EPL}, 91(6):6002, 2010.

\bibitem{Yeomans_20}
R~Hennings-Yeomans, C.~L. Chang, J.~Ding, et~al.
\newblock Controlling {Tc} of iridium films using the proximity effect.
\newblock {\em Journal of Applied Physics}, 128:154501, 2020.

\bibitem{Hertel_19}
S.~A. Hertel, A.~Biekert, J.~Lin, V.~Velan, and D.~N. McKinsey.
\newblock Direct detection of {sub-GeV} dark matter using a superfluid {$^4$He}
  target.
\newblock {\em Phys. Rev. D}, 100:092007, 2019.

\bibitem{hitlin2021progress}
David Hitlin.
\newblock Progress on a photosensor for the readout of the fast scintillation
  light component of {BaF$_2$}.
\newblock In {\em CPAD Instrumentation Frontier Workshop}, Stony Brook, NY, May
  2021.

\bibitem{Hochberg2019}
Yonit Hochberg, Ilya Charaev, Sae-Woo Nam, Varun Verma, Marco Colangelo, and
  Karl~K. Berggren.
\newblock Detecting sub-gev dark matter with superconducting nanowires.
\newblock {\em Phys. Rev. Lett.}, 123:151802, Oct 2019.

\bibitem{Hoenk1992_UVCCD_Delta}
Michael~E. Hoenk, Paula~J. Grunthaner, Frank~J. Grunthaner, R.~W. Terhune,
  Masoud Fattahi, and Hsin-Fu Tseng.
\newblock Growth of a delta-doped silicon layer by molecular beam epitaxy on a
  charge-coupled device for reflection-limited ultraviolet quantum efficiency.
\newblock {\em Applied Physics Letters}, 61(9):1084--1086, 1992.

\bibitem{Holland_2003}
S.~E. {Holland}, D.~E. {Groom}, N.~P. {Palaio}, R.~J. {Stover}, and {Mingzhi
  Wei}.
\newblock Fully depleted, back-illuminated charge-coupled devices fabricated on
  high-resistivity silicon.
\newblock {\em IEEE Transactions on Electron Devices}, 50(1):225--238, 2003.

\bibitem{Horns_13}
D.~Horns, J.~Jaeckel, A.~Lindner, et~al.
\newblock Searching for {WISPy} cold dark matter with a dish antenna.
\newblock {\em JCAP}, 04:016, 2013.

\bibitem{Igarashi:2015cma}
T.~Igarashi, M.~Tanaka, T.~Washimi, and K.~Yorita.
\newblock {Performance of VUV-sensitive MPPC for Liquid Argon Scintillation
  Light}.
\newblock {\em Nucl. Instrum. Meth.}, A833:239--244, 2016.

\bibitem{broadcom_nirenhancedsipm}
Broadcom Inc.
\newblock Broadcom's nir sipm technology sets new performance standards for
  lidar.
\newblock
  \textsc{url:}~\url{https://www.broadcom.com/blog/broadcoms-nir-sipm-technology-sets-performance-standards-for-lidar},
  February 2020.

\bibitem{Irwin_05}
K.~D. Irwin and G.~C. Hilton.
\newblock {\em "Transition-Edge Sensors" in Cryoegenic Particle Detection,
  Edited by C. Enss.}
\newblock Springer, 2005.

\bibitem{itzler2010design}
Mark~A Itzler, Mark Entwistle, Mark Owens, Ketan Patel, Xudong Jiang, Krystyna
  Slomkowski, Sabbir Rangwala, Peter~F Zalud, Tom Senko, John Tower, et~al.
\newblock Design and performance of single photon hep focal plane arrays for
  3-d ladar imaging.
\newblock In {\em Detectors and Imaging Devices: Infrared, Focal Plane, Single
  Photon}, volume 7780, page 77801M. International Society for Optics and
  Photonics, 2010.

\bibitem{Izhnin2021}
Ihor~I. Izhnin, Kirill~A. Lozovoy, Andrey~P. Kokhanenko, Kristina~I.
  Khomyakova, Rahaf M.~H. Douhan, Vladimir~V. Dirko, Alexander~V.
  Voitsekhovskii, Olena~I. Fitsych, and Nataliya~Yu. Akimenko.
\newblock Single-photon avalanche diode detectors based on group {IV}
  materials.
\newblock {\em Applied Nanoscience}, February 2021.

\bibitem{jamil2018vuv}
A.~Jamil, T.~Ziegler, P.~Hufschmidt, G.~Li, L.~Lupin-Jimenez, T.~Michel,
  I.~Ostrovskiy, F.~Retière, J.~Schneider, M.~Wagenpfeil, A.~Alamre, J.~B.
  Albert, G.~Anton, I.~J. Arnquist, I.~Badhrees, P.~S. Barbeau, D.~Beck,
  V.~Belov, T.~Bhatta, F.~Bourque, J.~P. Brodsky, E.~Brown, T.~Brunner,
  A.~Burenkov, G.~F. Cao, L.~Cao, W.~R. Cen, C.~Chambers, S.~A. Charlebois,
  M.~Chiu, B.~Cleveland, M.~Coon, M.~Côté, A.~Craycraft, W.~Cree,
  J.~Dalmasson, T.~Daniels, L.~Darroch, S.~J. Daugherty, J.~Daughhetee,
  S.~Delaquis, A.~Der Mesrobian-Kabakian, R.~DeVoe, J.~Dilling, Y.~Y. Ding,
  M.~J. Dolinski, A.~Dragone, J.~Echevers, L.~Fabris, D.~Fairbank, W.~Fairbank,
  J.~Farine, S.~Feyzbakhsh, R.~Fontaine, D.~Fudenberg, G.~Gallina,
  G.~Giacomini, R.~Gornea, G.~Gratta, E.~V. Hansen, D.~Harris, M.~Hasan,
  M.~Heffner, J.~H{\"o}{\ss}l, E.~W. Hoppe, A.~House, M.~Hughes, Y.~Ito,
  A.~Iverson, C.~Jessiman, M.~J. Jewell, X.~S. Jiang, A.~Karelin, L.~J.
  Kaufman, T.~Koffas, S.~Kravitz, R.~Krücken, A.~Kuchenkov, K.~S. Kumar,
  Y.~Lan, A.~Larson, D.~S. Leonard, S.~Li, Z.~Li, C.~Licciardi, Y.~H. Lin,
  P.~Lv, R.~MacLellan, B.~Mong, D.~C. Moore, K.~Murray, R.~J. Newby, Z.~Ning,
  O.~Njoya, F.~Nolet, O.~Nusair, K.~Odgers, A.~Odian, M.~Oriunno, J.~L. Orrell,
  G.~S. Ortega, C.~T. Overman, S.~Parent, A.~Piepke, A.~Pocar, J.-F. Pratte,
  D.~Qiu, V.~Radeka, E.~Raguzin, T.~Rao, S.~Rescia, A.~Robinson, T.~Rossignol,
  P.~C. Rowson, N.~Roy, R.~Saldanha, S.~Sangiorgio, S.~Schmidt, A.~Schubert,
  D.~Sinclair, K.~Skarpaas, A.~K. Soma, G.~St-Hilaire, V.~Stekhanov,
  T.~Stiegler, X.~L. Sun, M.~Tarka, J.~Todd, T.~Tolba, T.~I. Totev, R.~Tsang,
  T.~Tsang, F.~Vachon, B.~Veenstra, V.~Veeraraghavan, G.~Visser, J.-L.
  Vuilleumier, Q.~Wang, J.~Watkins, M.~Weber, W.~Wei, L.~J. Wen, U.~Wichoski,
  G.~Wrede, S.~X. Wu, W.~H. Wu, Q.~Xia, L.~Yang, Y.-R. Yen, O.~Zeldovich,
  X.~Zhang, J.~Zhao, and Y.~Zhou.
\newblock Vuv-sensitive silicon photomultipliers for xenon scintillation light
  detection in nexo.
\newblock {\em IEEE Transactions on Nuclear Science}, 65(11):2823--2833, 2018.

\bibitem{Janesick1988}
James Janesick, Tom Elliott, Richard Bredthauer, Charles Chandler, and Barry
  Burke.
\newblock {Fano-Noise-Limited CCDs}.
\newblock In Leon Golub, editor, {\em X-Ray Instrumentation in Astronomy II},
  volume 0982, pages 70 -- 95. International Society for Optics and Photonics,
  SPIE, 1988.

\bibitem{Kasap_2011}
Safa Kasap, Joel~B. Frey, George Belev, Olivier Tousignant, Habib Mani,
  Jonathan Greenspan, Luc Laperriere, Oleksandr Bubon, Alla Reznik, Giovanni
  DeCrescenzo, and et~al.
\newblock Amorphous and polycrystalline photoconductors for direct conversion
  flat panel x-ray image sensors.
\newblock {\em Sensors}, 11(5):5112–5157, May 2011.

\bibitem{Keimer2015}
B.~Keimer, S.~A. Kivelson, M.~R. Norman, S.~Uchida, and J.~Zaanen.
\newblock From quantum matter to high-temperature superconductivity in copper
  oxides.
\newblock {\em Nature}, 518(7538):179--186, Feb 2015.

\bibitem{1997-Kindt_SPAD-array}
W.~J. Kindt and H.~W. {van Zeijl}.
\newblock Fabrication of {{Geiger}} mode avalanche photodiodes.
\newblock In {\em 1997 {{IEEE}} nuclear science symposium conference record},
  pages 334--338 vol.1, {Albuquerque, USA}, 1997.

\bibitem{1999-Kindt_thesis}
W.J. Kindt.
\newblock {\em Geiger mode avalanche photodiode arrays: {{For}} spatially
  resolved single photon counting}.
\newblock {Delft University Press}, 1999.

\bibitem{1998-Kindt_SPAD-CMOS}
W.J. Kindt and H.W. {van Zeijl}.
\newblock Modelling and fabrication of {{Geiger}} mode avalanche photodiodes.
\newblock {\em IEEE Transactions on Nuclear Science}, 45:715--719, 1998.

\bibitem{Korneeva2018}
Yu.~P. Korneeva, D.~Yu. Vodolazov, A.~V. Semenov, I.~N. Florya, N.~Simonov,
  E.~Baeva, A.~A. Korneev, G.~N. Goltsman, and T.~M. Klapwijk.
\newblock Optical single-photon detection in micrometer-scale nbn bridges.
\newblock {\em Phys. Rev. Applied}, 9:064037, Jun 2018.

\bibitem{Korzh:2018}
B.~Korzh, Qingyuan Zhao, Simone Frasca, J.~Allmaras, T.~Autry, Eric Bersin,
  Marco Colangelo, G.~Crouch, Andrew Dane, T.~Gerrits, F.~Marsili, Galan Moody,
  E.~Ramirez, J.~Rezac, Martin Stevens, E.~Wollman, D.~Zhu, P.~Hale, Kevin
  Silverman, and Karl Berggren.
\newblock Demonstrating sub-3 ps temporal resolution in a superconducting
  nanowire single-photon detector.
\newblock {\em Nat. Photonics}, 14:250–255, 04 2018.

\bibitem{Kuzmenko2020}
Kateryna Kuzmenko, Peter Vines, Abderrahim Halimi, Robert~J. Collins, Aurora
  Maccarone, Aongus McCarthy, Zo\"{e}~M. Greener, Jaros{\l}aw Kirdoda, Derek
  C.~S. Dumas, Lourdes~Ferre Llin, Muhammad~M. Mirza, Ross~W. Millar,
  Douglas~J. Paul, and Gerald~S. Buller.
\newblock 3d lidar imaging using ge-on-si single-photon avalanche diode
  detectors.
\newblock {\em Opt. Express}, 28(2):1330--1344, Jan 2020.

\bibitem{doi:10.1021/acsphotonics.9b00012}
Andy LaBella, Jann Stavro, Sebastien Léveillé, Wei Zhao, and Amir~H. Goldan.
\newblock Picosecond time resolution with avalanche amorphous selenium.
\newblock {\em ACS Photonics}, 6(6):1338--1344, 2019.

\bibitem{lacaita1995performance}
A.~Lacaita, S.~Cova, C.~Samori, and M.~Ghioni.
\newblock Performance optimization of active quenching circuits for picosecond
  timing with single photon avalanche diodes.
\newblock {\em Review of scientific instruments}, 66(8):4289--4295, 1995.

\bibitem{Lawrie:2021}
Benjamin~J. Lawrie, Claire~E. Marvinney, Yun-Yi Pai, Matthew~A. Feldman, Jie
  Zhang, Aaron~J. Miller, Chengyun Hua, Eugene Dumitrescu, and G\'abor~B.
  Hal\'asz.
\newblock Multifunctional superconducting nanowire quantum sensors.
\newblock {\em Phys. Rev. Applied}, 16:064059, Dec 2021.

\bibitem{lee2017back}
M-J Lee, AR~Ximenes, P~Padmanabhan, TJ~Wang, KC~Huang, Y~Yamashita, DN~Yaung,
  and E~Charbon.
\newblock A back-illuminated 3d-stacked single-photon avalanche diode in 45nm
  cmos technology.
\newblock In {\em 2017 IEEE International Electron Devices Meeting (IEDM)},
  pages 16--6. IEEE, 2017.

\bibitem{Leitz2018}
C.~Leitz et~al.
\newblock {Development of germanium charge-coupled devices}.
\newblock In Andrew~D. Holland and James Beletic, editors, {\em High Energy,
  Optical, and Infrared Detectors for Astronomy VIII, SPIE Astronomical
  Telescopes + Instrumentation, 2018, Austin, Texas, United States}, volume
  10709, pages 1070908--1--7. International Society for Optics and Photonics,
  SPIE, 2018.

\bibitem{Leitz2019}
C.~Leitz et~al.
\newblock {Towards megapixel-class germanium charge-coupled devices for
  broadband x-ray detectors}.
\newblock In Oswald~H. Siegmund, editor, {\em UV, X-Ray, and Gamma-Ray Space
  Instrumentation for Astronomy XXI}, volume 11118, pages 111802--2--8.
  International Society for Optics and Photonics, SPIE, 2019.

\bibitem{Leitz2020}
C.~Leitz et~al.
\newblock {Germanium charge-coupled devices for hard x-ray astronomy}.
\newblock In Andrew~D. Holland and James Beletic, editors, {\em X-Ray, Optical,
  and Infrared Detectors for Astronomy IX, SPIE Astronomical Telescopes +
  Instrumentation, 2020, Online Only}, volume 11454, pages 114541B--1--8.
  International Society for Optics and Photonics, SPIE, 2020.

\bibitem{levine1984near}
BF~Levine, CG~Bethea, and JC~Campbell.
\newblock Near room temperature 1.3 $\mu$m single photon counting with a ingaas
  avalanche photodiode.
\newblock {\em Electronics Letters}, 20(14):596--598, 1984.

\bibitem{lindblom1988}
P.~Lindblom and A.~Solin.
\newblock Atomic near-infrared noble gas scintillation i optical spectra.
\newblock {\em Nucl. Instr. Meth.}, A268:204--208, 1988.

\bibitem{Litaa_08}
A.~E. Lita, A.~J. Miller, and S.~W. Nam.
\newblock Counting near-infrared single-photons with 95\% efficiency.
\newblock {\em Opt. Express}, 16:3032--3040, 2008.

\bibitem{Liu_21}
J.~Liu, K.~Dona, G.~Hoshino, et~al.
\newblock Broadband solenoidal haloscope for terahertz axion detection.
\newblock arXiv:2111.12103, 2021.

\bibitem{liu2021broadband}
Jesse Liu, Kristin Dona, Gabe Hoshino, Stefan Knirck, Noah Kurinsky, Matthew
  Malaker, David Miller, Andrew Sonnenschein, Pete Barry, Karl~K Berggren,
  et~al.
\newblock Broadband solenoidal haloscope for terahertz axion detection.
\newblock {\em arXiv preprint arXiv:2111.12103}, 2021.

\bibitem{Llin2020}
Lourdes~Ferre Llin, Jaros{\l}aw Kirdoda, Fiona Thorburn, Laura~L. Huddleston,
  Zo\"{e}~M. Greener, Kateryna Kuzmenko, Peter Vines, Derek C.~S. Dumas,
  Ross~W. Millar, Gerald~S. Buller, and Douglas~J. Paul.
\newblock High sensitivity ge-on-si single-photon avalanche diode detectors.
\newblock {\em Opt. Lett.}, 45(23):6406--6409, Dec 2020.

\bibitem{llin2020high}
Lourdes~Ferre Llin, Jaros{\l}aw Kirdoda, Fiona Thorburn, Laura~L Huddleston,
  Zo{\"e}~M Greener, Kateryna Kuzmenko, Peter Vines, Derek~CS Dumas, Ross~W
  Millar, Gerald~S Buller, et~al.
\newblock High sensitivity ge-on-si single-photon avalanche diode detectors.
\newblock {\em Optics Letters}, 45(23):6406--6409, 2020.

\bibitem{losero2018unbiased}
Elena Losero, Ivano Ruo-Berchera, Alice Meda, Alessio Avella, and Marco
  Genovese.
\newblock Unbiased estimation of an optical loss at the ultimate quantum limit
  with twin-beams.
\newblock {\em Scientific reports}, 8(1):1--11, 2018.

\bibitem{lu2011geiger}
Zhiwen Lu, Yimin Kang, Chong Hu, Qiugui Zhou, Han-Din Liu, and Joe~C Campbell.
\newblock Geiger-mode operation of ge-on-si avalanche photodiodes.
\newblock {\em IEEE Journal of Quantum Electronics}, 47(5):731--735, 2011.

\bibitem{ma20154mp}
Cheng Ma, Yang Liu, Jing Li, Quan Zhou, Yuchun Chang, and Xinyang Wang.
\newblock A 4mp high-dynamic-range, low-noise cmos image sensor.
\newblock In {\em Image Sensors and Imaging Systems 2015}, volume 9403, page
  940305. International Society for Optics and Photonics, 2015.

\bibitem{Quanta_Fossum}
Jiaju Ma, Saleh Masoodian, Yue Song, Kofi Odame, Eric Fossum, and Donald
  Hondongwa.
\newblock Quanta image sensor (qis): Early research progress.
\newblock In {\em Optics InfoBase Conference Papers}, 06 2013.

\bibitem{Quanta_camera}
Jiaju Ma, Dexue Zhang, Omar~A. Elgendy, and Saleh Masoodian.
\newblock A 0.19e- rms read noise 16.7mpixel stacked quanta image sensor with
  1.1 $\mu$m-pitch backside illuminated pixels.
\newblock {\em IEEE Electron Device Letters}, 42(6):891--894, 2021.

\bibitem{Magnoni:21}
Agustina~G. Magnoni, Muriel Bonetto, Juan Estrada, Miguel~A. Larotonda, and
  Dario Rodrigues.
\newblock Sub-shot noise absorption measurements using a skipper-ccd and
  twin-beams: a work in progress.
\newblock In {\em Quantum Information and Measurement VI 2021}, page W2B.5.
  Optical Society of America, 2021.

\bibitem{marcelot2014study}
Olivier Marcelot, Magali Estribeau, Vincent Goiffon, Philippe Martin-Gonthier,
  Franck Corbi{\`e}re, Romain Molina, S{\'e}bastien Rolando, and Pierre Magnan.
\newblock Study of ccd transport on cmos imaging technology: Comparison between
  sccd and bccd, and ramp effect on the cti.
\newblock {\em IEEE Transactions on Electron Devices}, 61(3):844--849, 2014.

\bibitem{2019BAAS...51g.126M}
Jennifer {Marshall}, Adam {Bolton}, James {Bullock}, Adam {Burgasser}, Ken
  {Chambers}, Darren {DePoy}, Arjun {Dey}, Nicolas {Flagey}, Alexis {Hill},
  Lynne {Hillenbrand}, Daniel {Huber}, Ting {Li}, Stephanie {Juneau}, Manoj
  {Kaplinghat}, Mario {Mateo}, Alan {McConnachie}, Jeffrey {Newman}, Andreea
  {Petric}, David {Schlegel}, Andrew {Sheinis}, Yue {Shen}, Doug {Simons},
  Michael {Strauss}, Kei {Szeto}, Kim-Vy {Tran}, and Christophe {Y{\`e}che}.
\newblock {The Maunakea Spectroscopic Explorer}.
\newblock In {\em Bulletin of the American Astronomical Society}, volume~51,
  page 126, September 2019.

\bibitem{martinez2017single}
Nicholas~JD Martinez, Michael Gehl, Christopher~T Derose, Andrew~L Starbuck,
  Andrew~T Pomerene, Anthony~L Lentine, Douglas~C Trotter, and Paul~S Davids.
\newblock Single photon detection in a waveguide-coupled ge-on-si lateral
  avalanche photodiode.
\newblock {\em Optics express}, 25(14):16130--16139, 2017.

\bibitem{Mattis:1958vo}
D~C Mattis and J~Bardeen.
\newblock {Theory of the Anomalous Skin Effect in Normal and Superconducting
  Metals}.
\newblock {\em Physical Review}, 111(2):412--417, 1958.

\bibitem{mazzillo2012electro}
Massimo Mazzillo, Anatoly Ronzhin, Sergey Los, Salvatore Abbisso, Delfo
  Sanfilippo, Giusy Valvo, Beatrice Carbone, Angelo Piana, Giorgio Fallica,
  Michael Albrow, et~al.
\newblock Electro-optical performances of p-on-n and n-on-p silicon
  photomultipliers.
\newblock {\em IEEE transactions on electron devices}, 59(12):3419--3425, 2012.

\bibitem{2012RScI...83d4702M}
Sean McHugh, Benjamin~A Mazin, Bruno Serfass, Seth Meeker, Kieran O'Brien, Ran
  Duan, Rick Raffanti, and Dan Werthimer.
\newblock {A readout for large arrays of microwave kinetic inductance
  detectors}.
\newblock {\em Review of Scientific Instruments}, 83(4):4702, April 2012.

\bibitem{mcintosh2002ingaasp}
KA~McIntosh, JP~Donnelly, DC~Oakley, A~Napoleone, SD~Calawa, LJ~Mahoney,
  KM~Molvar, EK~Duerr, SH~Groves, and DC~Shaver.
\newblock Ingaasp/inp avalanche photodiodes for photon counting at 1.06 $\mu$m.
\newblock {\em Applied Physics Letters}, 81(14):2505--2507, 2002.

\bibitem{mclntosh2003arrays}
KA~Mclntosh, JP~Donnelly, DC~Oakley, A~Napoleone, SD~Calawa, LJ~Mahoney,
  KM~Molvar, J~Mahan, RJ~Molnar, EK~Duerr, et~al.
\newblock Arrays of iii-v semiconductor geiger-mode avalanche photodiodes.
\newblock In {\em The 16th Annual Meeting of the IEEE Lasers and Electro-Optics
  Society, 2003. LEOS 2003.}, volume~2, pages 686--687. IEEE, 2003.

\bibitem{habex}
Bertrand {Mennesson}, Scott {Gaudi}, Sara {Seager}, Alina {Kiessling}, and
  Keith {Warfield}.
\newblock {The Habitable Exoplanet Observatory mission concept}.
\newblock In {\em Society of Photo-Optical Instrumentation Engineers (SPIE)
  Conference Series}, volume 11443 of {\em Society of Photo-Optical
  Instrumentation Engineers (SPIE) Conference Series}, page 1144320, December
  2020.

\bibitem{Mitrano-sa-2019}
Matteo Mitrano, Sangjun Lee, Ali~A. Husain, Luca Delacretaz, Minhui Zhu,
  Gilberto de~la Peña~Munoz, Stella X.-L. Sun, Young~Il Joe, Alexander~H.
  Reid, Scott~F. Wandel, Giacomo Coslovich, William Schlotter, Tim van Driel,
  John Schneeloch, G.~D. Gu, Sean Hartnoll, Nigel Goldenfeld, and Peter
  Abbamonte.
\newblock Ultrafast time-resolved x-ray scattering reveals diffusive charge
  order dynamics in
  la<sub>2\&\#x2013;<i>x</i></sub>ba<i><sub>x</sub></i>cuo<sub>4</sub>.
\newblock {\em Science Advances}, 5(8):eaax3346, 2019.

\bibitem{moreau2019imaging}
Paul-Antoine Moreau, Ermes Toninelli, Thomas Gregory, and Miles~J Padgett.
\newblock Imaging with quantum states of light.
\newblock {\em Nature Reviews Physics}, 1(6):367--380, 2019.

\bibitem{Nagler_18}
P.~C. Nagler, M.~A. Greenhouse, S.~H. Moseley, et~al.
\newblock Development of transition edge sensor detectors optimized for
  single-photon spectroscopy in the optical and near-infrared.
\newblock {\em Proc. SPIE}, 10709:1070931, 2018.

\bibitem{Nagler_21}
P.~C. Nagler, J.~E. Sadleir, and E.~J. Wollack.
\newblock Transition-edge sensor detectors for the origins space telescope.
\newblock {\em J. of Astronomical Telescopes, Instruments, and Systems},
  7(1):011005, 2021.

\bibitem{Nakano2012}
S.~Nakano, Y.~Takeuchi, T.~Kaneko, and M.~Kondo.
\newblock Influence of surface treatments on crystalline germanium
  heterojunction solar cell characteristics.
\newblock {\em Journal of Non-Crystalline Solids}, 358(17):2249--2252, 2012.

\bibitem{Nakarmi_2020}
P.~Nakarmi, I.~Ostrovskiy, A.K. Soma, F.~Reti{\`{e}}re, S.~Al Kharusi,
  M.~Alfaris, G.~Anton, I.J. Arnquist, I.~Badhrees, P.S. Barbeau, D.~Beck,
  V.~Belov, T.~Bhatta, J.~Blatchford, P.A. Breur, J.P. Brodsky, E.~Brown,
  T.~Brunner, S.~Byrne Mamahit, E.~Caden, G.F. Cao, L.~Cao, C.~Chambers,
  B.~Chana, S.A. Charlebois, M.~Chiu, B.~Cleveland, M.~Coon, A.~Craycraft,
  J.~Dalmasson, T.~Daniels, L.~Darroch, A.~De~St. Croix, A.~Der
  Mesrobian-Kabakian, R.~DeVoe, M.L.~Di Vacri, J.~Dilling, Y.Y. Ding, M.J.
  Dolinski, L.~Doria, A.~Dragone, J.~Echevers, F.~Edaltafar, M.~Elbeltagi,
  L.~Fabris, D.~Fairbank, W.~Fairbank, J.~Farine, S.~Ferrara, S.~Feyzbakhsh,
  R.~Fontaine, A.~Fucarino, G.~Gallina, P.~Gautam, G.~Giacomini, D.~Goeldi,
  R.~Gornea, G.~Gratta, E.V. Hansen, M.~Heffner, E.W. Hoppe, J.~H{\"o}{\ss}l,
  A.~House, M.~Hughes, A.~Iverson, A.~Jamil, M.J. Jewell, X.S. Jiang,
  A.~Karelin, L.J. Kaufman, T.~Koffas, R.~Kr{\"u}cken, A.~Kuchenkov, K.S.
  Kumar, Y.~Lan, A.~Larson, K.G. Leach, B.G. Lenardo, D.S. Leonard, G.~Li,
  S.~Li, Z.~Li, C.~Licciardi, P.~Lv, R.~MacLellan, N.~Massacret, T.~McElroy,
  M.~Medina-Peregrina, T.~Michel, B.~Mong, D.C. Moore, K.~Murray, C.R. Natzke,
  R.J. Newby, Z.~Ning, O.~Njoya, F.~Nolet, O.~Nusair, K.~Odgers, A.~Odian,
  M.~Oriunno, J.L. Orrell, G.S. Ortega, C.T. Overman, S.~Parent, A.~Piepke,
  A.~Pocar, J.-F. Pratte, V.~Radeka, E.~Raguzin, S.~Rescia, M.~Richman,
  A.~Robinson, T.~Rossignol, P.C. Rowson, N.~Roy, J.~Runge, R.~Saldanha,
  S.~Sangiorgio, K.~Skarpaas VIII, G.~St-Hilaire, V.~Stekhanov, T.~Stiegler,
  X.L. Sun, M.~Tarka, J.~Todd, T.I. Totev, R.~Tsang, T.~Tsang, F.~Vachon,
  V.~Veeraraghavan, S.~Viel, G.~Visser, C.~Vivo-Vilches, J.-L. Vuilleumier,
  M.~Wagenpfeil, T.~Wager, M.~Walent, Q.~Wang, M.~Ward, J.~Watkins, M.~Weber,
  W.~Wei, L.J. Wen, U.~Wichoski, S.X. Wu, W.H. Wu, X.~Wu, Q.~Xia, H.~Yang,
  L.~Yang, O.~Zeldovich, J.~Zhao, Y.~Zhou, and T.~Ziegler.
\newblock Reflectivity and {PDE} of {VUV}4 hamamatsu {SiPMs} in liquid xenon.
\newblock {\em Journal of Instrumentation}, 15(01):P01019--P01019, jan 2020.

\bibitem{nanver2014robust}
Lis~K Nanver, Lin Qi, Vahid Mohammadi, KRM Mok, Wiebe~B de~Boer, Negin
  Golshani, Amir Sammak, Thomas~LM Scholtes, Alexander Gottwald, Udo Kroth,
  et~al.
\newblock Robust uv/vuv/euv pureb photodiode detector technology with high cmos
  compatibility.
\newblock {\em IEEE Journal of Selected Topics in Quantum Electronics},
  20(6):306--316, 2014.

\bibitem{Nasteva_2021}
Irina Nasteva.
\newblock Low-energy reactor neutrino physics with the connie experiment.
\newblock {\em Journal of Physics: Conference Series}, 2156(1):012115, Dec
  2021.

\bibitem{Decadal2020}
{National Academies of Sciences, Engineering, and Medicine}.
\newblock {\em {Pathways to Discovery in Astronomy and Astrophysics for the
  2020s}}.
\newblock 2021.

\bibitem{NeumeierEPL}
A.~Neumeier, T.~Dandl, T.~Heindl, A.~Himpsl, L.~Oberauer, W.~Potzel, S.~Roth,
  S.~Schönert, J.~Wieser, and A.~Ulrich.
\newblock Intense vacuum-ultraviolet and infrared scintillation of liquid ar-xe
  mixtures.
\newblock {\em EPL}, 109(1):12001, 2015.

\bibitem{2005-Niclass-Rochas-Charbon_CMOS-SPAD-camera-32x32-800nm}
Cristiano Niclass, Alexis Rochas, Pierre-Andre Besse, and Edoardo Charbon.
\newblock Design and characterization of a {{CMOS}} 3-{{D}} image sensor based
  on single photon avalanche diodes.
\newblock {\em IEEE Journal of Solid-State Circuits}, 40(9):1847--1854, 2005.

\bibitem{nikzad2012delta}
Shouleh Nikzad, Michael~E Hoenk, Frank Greer, Blake Jacquot, Steve Monacos,
  Todd~J Jones, Jordana Blacksberg, Erika Hamden, David Schiminovich, Chris
  Martin, et~al.
\newblock Delta-doped electron-multiplied ccd with absolute quantum efficiency
  over 50\% in the near to far ultraviolet range for single photon counting
  applications.
\newblock {\em Applied Optics}, 51(3):365--369, 2012.

\bibitem{BRN_19}
U.S.~Department of~Energy.
\newblock Basic research needs for dark-matter small projects new initiatives.
\newblock https://www.osti.gov/servlets/purl/1659757, 2019.

\bibitem{luvoir}
J.~{O'Meara} and {Luvoir Mission Concept Study Team}.
\newblock {The LUVOIR Mission Concept: Telling the Story of Life in the
  Universe}.
\newblock In {\em American Astronomical Society Meeting Abstracts \#235},
  volume 235 of {\em American Astronomical Society Meeting Abstracts}, page
  447.04, January 2020.

\bibitem{onsemi_nirenhancedsipm}
onsemi.
\newblock Rb-series sipm: Silicon photomultipliers, nir-enhanced.
\newblock
  \textsc{url:}~\url{https://www.onsemi.com/products/sensors/photodetectors-sipm-spad/silicon-photomultipliers-sipm/rb-series-sipm},
  March 2022.

\bibitem{organtini2020industrial}
Paolo Organtini, Alberto Gola, Giovanni Paternoster, Fabio Acerbi, Giovanni
  Margutti, and Roberto Bez.
\newblock Industrial exploitation of sipm technology developed for basic
  research.
\newblock {\em Nuclear Instruments and Methods in Physics Research Section A:
  Accelerators, Spectrometers, Detectors and Associated Equipment}, 978:164410,
  2020.

\bibitem{Paoluccii_20}
F.~Paolucci, V.~Buccheri, G.~Germanese, et~al.
\newblock Development of highly sensitive nanoscale transition edge sensors for
  gigahertz astronomy and dark matter search.
\newblock {\em J. Appl. Phys.}, 128:194502, 2020.

\bibitem{paternoster2019silicon}
Giovanni Paternoster, Lorenza Ferrario, Fabio Acerbi, Alberto~Giacomo Gola, and
  Pierluigi Bellutti.
\newblock Silicon photomultipliers technology at fondazione bruno kessler and
  3d integration perspectives.
\newblock In {\em ESSDERC 2019-49th European Solid-State Device Research
  Conference (ESSDERC)}, pages 50--53. IEEE, 2019.

\bibitem{podmore2021qkd}
H~Podmore, I~D'Souza, J~Cain, T~Jennewein, BL~Higgins, YS~Lee, A~Koujelev,
  D~Hudson, and A~McColgan.
\newblock Qkd terminal for canada’s quantum encryption and science satellite
  (qeyssat).
\newblock In {\em International Conference on Space Optics—ICSO 2020}, volume
  11852, page 118520H. International Society for Optics and Photonics, 2021.

\bibitem{Polakovic2020}
Tomas Polakovic, Whitney Armstrong, Volodymyr Yefremenko, John~E. Pearson,
  Kawtar Hafidi, Goran Karapetrov, Zein-Eddine Meziani, and Valentyn Novosad.
\newblock Superconducting nanowires as high-rate photon detectors in strong
  magnetic fields.
\newblock {\em Nuclear Instruments \& Methods in Physics Research Section
  A-accelerators Spectrometers Detectors and Associated Equipment}, 959:163543,
  2020.

\bibitem{Posthuma2003}
N.E. Posthuma, G.~Flamand, and J.~Poortmans.
\newblock {Development of standalone germanium solar cells for application in
  space using spin-on diffusants}.
\newblock In {\em Proceedings 3rd World Conference Photovoltaic Energy
  Conversion, Osaka, Japan}, volume~1, page 777–780, 2003.

\bibitem{Pratte2021_Sensors}
Jean-Fran{\c{c}}ois Pratte, Fr{\'e}d{\'e}ric Nolet, Samuel Parent,
  Fr{\'e}d{\'e}ric Vachon, Nicolas Roy, Tommy Rossignol, Keven Deslandes, Henri
  Dautet, R{\'e}jean Fontaine, and Serge~A Charlebois.
\newblock 3d photon-to-digital converter for radiation instrumentation:
  Motivation and future works.
\newblock {\em Sensors}, 21(2), 2021.

\bibitem{ravindran2020active}
Prasana Ravindran, Risheng Cheng, Hong Tang, and Joseph~C Bardin.
\newblock Active quenching of superconducting nanowire single photon detectors.
\newblock {\em Optics express}, 28(3):4099--4114, 2020.

\bibitem{Reddy:2020}
Dileep~V. Reddy, Robert~R. Nerem, Sae~Woo Nam, Richard~P. Mirin, and Varun~B.
  Verma.
\newblock Superconducting nanowire single-photon detectors with 98\% system
  detection efficiency at 1550nm.
\newblock {\em Optica}, 7(12):1649--1653, Dec 2020.

\bibitem{Richmond:2020}
Michael~W. {Richmond}, Masaomi {Tanaka}, Tomoki {Morokuma}, Shigeyuki {Sako},
  Ryou {Ohsawa}, Noriaki {Arima}, Nozomu {Tominaga}, Mamoru {Doi}, Tsutomu
  {Aoki}, Ko~{Arimatsu}, Makoto {Ichiki}, Shiro {Ikeda}, Yoshifusa {Ita},
  Toshihiro {Kasuga}, Koji~S. {Kawabata}, Hideyo {Kawakita}, Naoto {Kobayashi},
  Mitsuru {Kokubo}, Masahiro {Konishi}, Hiroyuki {Maehara}, Hiroyuki {Mito},
  Takashi {Miyata}, Yuki {Mori}, Mikio {Morii}, Kentaro {Motohara}, Yoshikazu
  {Nakada}, Shin-Ichiro {Okumura}, Hiroki {Onozato}, Yuki {Sarugaku}, Mikiya
  {Sato}, Toshikazu {Shigeyama}, Takao {Soyano}, Hidenori {Takahashi}, Ataru
  {Tanikawa}, Ken'ichi {Tarusawa}, Seitaro {Urakawa}, Fumihiko {Usui}, Junichi
  {Watanabe}, Takuya {Yamashita}, and Makoto {Yoshikawa}.
\newblock {An optical search for transients lasting a few seconds}.
\newblock {\em Publications of the Astronomical Society of Japan}, 72(1):3,
  February 2020.

\bibitem{2003-Rochas_SPAD-CMOS}
A.~Rochas, M.~Gani, B.~Furrer, P.A. Besse, R.S. Popovic, G.~Ribordy, and
  N.~Gisin.
\newblock Single photon detector fabricated in a complementary
  metal-oxide-semiconductor high-voltage technology.
\newblock {\em Review of Scientific Instruments}, 74(7):3263--3270, 2003.

\bibitem{Rochas2DSiPM}
A.~Rochas, M.~Gosch, A.~Serov, P.~A. Besse, R.~S. Popovic, T.~Lasser, and
  R.~Rigler.
\newblock First fully integrated 2-{{D}} array of single-photon detectors in
  standard {{CMOS}} technology.
\newblock {\em IEEE Photonics Technology Letters}, 15(7):963--965, 2003.

\bibitem{2003-Rochas_thesis}
Alexis Rochas.
\newblock {\em Single photon avalanche diodes in {{CMOS}} technology}.
\newblock {EPFL}, {Lausanne}, 2003.

\bibitem{rodrigues2020absolute}
Dario Rodrigues, Kevin Andersson, Mariano Cababie, Andre Donadon, Gustavo
  Cancelo, Juan Estrada, Guillermo Fernandez-Moroni, Ricardo Piegaia, Matias
  Senger, Miguel~Sofo Haro, et~al.
\newblock Absolute measurement of the fano factor using a skipper-ccd.
\newblock {\em arXiv preprint arXiv:2004.11499}, 2020.

\bibitem{Rosenberg_07}
D.~Rosenberg, J.~W. Harrington, P.~R. Rice, et~al.
\newblock Long-distance decoy-state quantum key distribution in optical fiber.
\newblock {\em Phys. Rev. Lett.}, 98:010503, 2007.

\bibitem{Rothe_18}
J.~Rothe, P.~Angloher, G.~Bauer, et~al.
\newblock {TES}-based light detectors for the {CRESST} direct dark matter
  search.
\newblock {\em J Low Temp Phys}, 193:1160--1166, 2018.

\bibitem{Rubbia1977}
Carlo Rubbia.
\newblock The liquid argon time projection chamber: a new concept for neutrino
  detectors.
\newblock Technical report, {CERN}, 1977.

\bibitem{Saab_phd2002}
T.~Saab.
\newblock {\em Searching for Weakly Interacting Particles with the Cryogenic
  Dark Matter Experiment}.
\newblock PhD thesis, Stanford University, 2002.

\bibitem{doi:10.1063/1.3579262}
Ichitaro Saito, Wataru Miyazaki, Masanori Onishi, Yuki Kudo, Tomoaki Masuzawa,
  Takatoshi Yamada, Angel Koh, Daniel Chua, Kenichi Soga, Mauro Overend, Masami
  Aono, Gehan A.~J. Amaratunga, and Ken Okano.
\newblock A transparent ultraviolet triggered amorphous selenium p-n junction.
\newblock {\em Applied Physics Letters}, 98(15):152102, 2011.

\bibitem{samantaray2017realization}
Nigam Samantaray, Ivano Ruo-Berchera, Alice Meda, and Marco Genovese.
\newblock Realization of the first sub-shot-noise wide field microscope.
\newblock {\em Light: Science \& Applications}, 6(7):e17005--e17005, 2017.

\bibitem{2000-Saveliev_first-SiPM}
V~Saveliev and V~Golovin.
\newblock Silicon avalanche photodiodes on the base of
  metal-resistor-semiconductor ({{MRS}}) structures.
\newblock {\em Nuclear Instruments and Methods in Physics Research Section A:
  Accelerators, Spectrometers, Detectors and Associated Equipment},
  442(1):223--229, 2000.

\bibitem{scarcella2014ingaas}
Carmelo Scarcella, Gianluca Boso, Alessandro Ruggeri, and Alberto Tosi.
\newblock Ingaas/inp single-photon detector gated at 1.3 ghz with 1.5\%
  afterpulsing.
\newblock {\em IEEE Journal of selected topics in quantum electronics},
  21(3):17--22, 2014.

\bibitem{2015-Charbon_dSiPM-review}
Dennis~R Schaart, Edoardo Charbon, Thomas Frach, and Volkmar Schulz.
\newblock Advances in digital {{SiPMs}} and their application in biomedical
  imaging.
\newblock {\em Nuclear Instruments and Methods in Physics Research Section A:
  Accelerators, Spectrometers, Detectors and Associated Equipment}, 809:31--52,
  2016.

\bibitem{MegaMapper}
David {Schlegel}, Juna~A. {Kollmeier}, and Simone {Ferraro}.
\newblock {The MegaMapper: a $z>2$ spectroscopic instrument for the study of
  Inflation and Dark Energy}.
\newblock In {\em Bulletin of the American Astronomical Society}, volume~51,
  page 229, September 2019.

\bibitem{Schroder1974}
D.~K. Schroder.
\newblock A two-phase germanium charge-coupled device.
\newblock {\em Applied Physics Letters}, 25:747, 1974.

\bibitem{schuette2011mbe}
Daniel~R Schuette, Richard~C Westhoff, Joseph~S Ciampi, Gayatri~E Perlin,
  Douglas~J Young, Brian~F Aull, Robert~K Reich, and David~C Shaver.
\newblock Mbe back-illuminated silicon geiger-mode avalanche photodiodes for
  enhanced ultraviolet response.
\newblock In {\em Advanced Photon Counting Techniques V}, volume 8033, page
  80330D. International Society for Optics and Photonics, 2011.

\bibitem{Seaberg-prl-2017}
M.~H. Seaberg, B.~Holladay, J.~C.~T. Lee, M.~Sikorski, A.~H. Reid, S.~A.
  Montoya, G.~L. Dakovski, J.~D. Koralek, G.~Coslovich, S.~Moeller, W.~F.
  Schlotter, R.~Streubel, S.~D. Kevan, P.~Fischer, E.~E. Fullerton, J.~L.
  Turner, F.-J. Decker, S.~K. Sinha, S.~Roy, and J.~J. Turner.
\newblock Nanosecond x-ray photon correlation spectroscopy on magnetic
  skyrmions.
\newblock {\em Phys. Rev. Lett.}, 119:067403, Aug 2017.

\bibitem{Seo2007}
Hokuto Seo, Satoshi Aihara, Toshihisa Watabe, Hiroshi Ohtake, Misao Kubota, and
  Norifumi Egami.
\newblock Color sensors with three vertically stacked organic photodetectors.
\newblock {\em Japanese Journal of Applied Physics}, 46(No. 49):L1240--L1242,
  dec 2007.

\bibitem{Shen-mrs-2021}
L.~Shen, M.~Seaberg, E.~Blackburn, and J.~J. Turner.
\newblock A snapshot review---fluctuations in quantum materials: from skyrmions
  to superconductivity.
\newblock {\em MRS Advances}, 6(8):221--233, May 2021.

\bibitem{signorelli2021low}
Fabio Signorelli, Fabio Telesca, Enrico Conca, Adriano Della~Frera, Alessandro
  Ruggeri, Andrea Giudice, and Alberto Tosi.
\newblock Low-noise ingaas/inp single-photon avalanche diodes for fiber-based
  and free-space applications.
\newblock {\em IEEE Journal of Selected Topics in Quantum Electronics},
  28(2):1--10, 2021.

\bibitem{skyrme-1962-nucphys}
T.H.R. Skyrme.
\newblock A unified field theory of mesons and baryons.
\newblock {\em Nuclear Physics}, 31:556 -- 569, 1962.

\bibitem{Sony3DCMOScamera}
{SONY}.
\newblock Sony develops next-generation back-illuminated {{CMOS}} image sensor
  which embodies the continuous evolution of the camera.

\bibitem{stefanov2020simulations}
Konstantin~D Stefanov, Martin~J Prest, Mark Downing, Elizabeth George, Naidu
  Bezawada, and Andrew~D Holland.
\newblock Simulations and design of a single-photon cmos imaging pixel using
  multiple non-destructive signal sampling.
\newblock {\em Sensors}, 20(7):2031, 2020.

\bibitem{Sze2007}
S.~M. Sze and Kwok~K. NG.
\newblock {\em Physics and Properties of Semiconductors}, chapter~1.
\newblock John Wiley \& Sons, Ltd, 2006.

\bibitem{Szypryt:2017cb}
P~Szypryt, S~R Meeker, G~Coiffard, N~Fruitwala, B~Bumble, G~Ulbricht, A~B
  Walter, M~Daal, C~Bockstiegel, G~Collura, N~Zobrist, I~Lipartito, and B~A
  Mazin.
\newblock {Large-format platinum silicide microwave kinetic inductance
  detectors for optical to near-IR astronomy}.
\newblock {\em Optics Express}, 25(21):25894--25909, 2017.

\bibitem{takai2016single}
Isamu Takai, Hiroyuki Matsubara, Mineki Soga, Mitsuhiko Ohta, Masaru Ogawa, and
  Tatsuya Yamashita.
\newblock Single-photon avalanche diode with enhanced nir-sensitivity for
  automotive lidar systems.
\newblock {\em Sensors}, 16(4):459, 2016.

\bibitem{taylor2016quantum}
Michael~A Taylor and Warwick~P Bowen.
\newblock Quantum metrology and its application in biology.
\newblock {\em Physics Reports}, 615:1--59, 2016.

\bibitem{taylor}
Michael~A Taylor, Jiri Janousek, Vincent Daria, Joachim Knittel, Boris Hage,
  Hans-A Bachor, and Warwick~P Bowen.
\newblock Biological measurement beyond the quantum limit.
\newblock {\em Nature Photonics}, 7(3):229--233, 2013.

\bibitem{excelitas_nirenhancedspad}
Excelitas Technologies.
\newblock Spcm-aqrh.
\newblock \textsc{url:}~\url{https://www.excelitas.com/product/spcm-aqrh},
  March 2022.

\bibitem{ccdProcess}
Teledyne-DALSA.
\newblock {CCD} foundry services.
\newblock
  \textsc{url:}~\url{https://www.teledynedalsa.com/en/products/foundry/ccd/},
  2019.

\bibitem{MSE19}
{The MSE Science Team}, Carine {Babusiaux}, Maria {Bergemann}, Adam
  {Burgasser}, Sara {Ellison}, Daryl {Haggard}, Daniel {Huber}, Manoj
  {Kaplinghat}, Ting {Li}, Jennifer {Marshall}, Sarah {Martell}, Alan
  {McConnachie}, Will {Percival}, Aaron {Robotham}, Yue {Shen}, Sivarani
  {Thirupathi}, Kim-Vy {Tran}, Christophe {Yeche}, David {Yong}, Vardan
  {Adibekyan}, Victor {Silva Aguirre}, George {Angelou}, Martin {Asplund},
  Michael {Balogh}, Projjwal {Banerjee}, Michele {Bannister}, Daniela
  {Barr{\'\i}a}, Giuseppina {Battaglia}, Amelia {Bayo}, Keith {Bechtol},
  Paul~G. {Beck}, Timothy~C. {Beers}, Earl~P. {Bellinger}, Trystyn {Berg},
  Joachim~M. {Bestenlehner}, Maciej {Bilicki}, Bertram {Bitsch}, Joss
  {Bland-Hawthorn}, Adam~S. {Bolton}, Alessandro {Boselli}, Jo~{Bovy}, Angela
  {Bragaglia}, Derek {Buzasi}, Elisabetta {Caffau}, Jan {Cami}, Timothy
  {Carleton}, Luca {Casagrande}, Santi {Cassisi}, M{\'a}rcio {Catelan}, Chihway
  {Chang}, Luca {Cortese}, Ivana {Damjanov}, Luke J.~M. {Davies}, Richard {de
  Grijs}, Gisella {de Rosa}, Alis {Deason}, Paola {di Matteo}, Alex
  {Drlica-Wagner}, Denis {Erkal}, Ana {Escorza}, Laura {Ferrarese}, Scott~W.
  {Fleming}, Andreu {Font-Ribera}, Ken {Freeman}, Boris~T. {G{\"a}nsicke},
  Maksim {Gabdeev}, Sarah {Gallagher}, Davide {Gandolfi}, Rafael~A.
  {Garc{\'\i}a}, Patrick {Gaulme}, Marla {Geha}, Mario {Gennaro}, Mark
  {Gieles}, Karoline {Gilbert}, Yjan {Gordon}, Aruna {Goswami}, Johnny~P.
  {Greco}, Carl {Grillmair}, Guillaume {Guiglion}, Vincent
  {H{\'e}nault-Brunet}, Patrick {Hall}, Gerald {Hand ler}, Terese {Hansen},
  Nimish {Hathi}, Despina {Hatzidimitriou}, Misha {Haywood}, Juan~V.
  {Hern{\'a}ndez Santisteban}, Lynne {Hillenbrand}, Andrew~M. {Hopkins}, Cullan
  {Howlett}, Michael~J. {Hudson}, Rodrigo {Ibata}, Dragana {Ili{\'c}}, Pascale
  {Jablonka}, Alexander {Ji}, Linhua {Jiang}, Stephanie {Juneau}, Amanda
  {Karakas}, Drisya {Karinkuzhi}, Stacy~Y. {Kim}, Xu~{Kong}, Iraklis
  {Konstantopoulos}, Jens-Kristian {Krogager}, Claudia {Lagos}, Rosine
  {Lallement}, Chervin {Laporte}, Yveline {Lebreton}, Khee-Gan {Lee},
  Geraint~F. {Lewis}, Sophia {Lianou}, Xin {Liu}, Nicolas {Lodieu}, Jon
  {Loveday}, Szabolcs {M{\'e}sz{\'a}ros}, Martin {Makler}, Yao-Yuan {Mao},
  Danilo {Marchesini}, Nicolas {Martin}, Mario {Mateo}, Carl {Melis}, Thibault
  {Merle}, Andrea {Miglio}, Faizan {Gohar Mohammad}, Karan {Molaverdikhani},
  Richard {Monier}, Thierry {Morel}, Benoit {Mosser}, David {Nataf}, Lina
  {Necib}, Hilding~R. {Neilson}, Jeffrey~A. {Newman}, A.~M. {Nierenberg}, Brian
  {Nord}, Pasquier {Noterdaeme}, Chris {O'Dea}, Mahmoudreza {Oshagh}, Andrew~B.
  {Pace}, Nathalie {Palanque-Delabrouille}, Gajendra {Pandey}, Laura~C.
  {Parker}, Marcel~S. {Pawlowski}, Annika H.~G. {Peter}, Patrick {Petitjean},
  Andreea {Petric}, Vinicius {Placco}, Luka~{\v{C}}. {Popovi{\'c}}, Adrian~M.
  {Price-Whelan}, Andrej {Prsa}, Swara {Ravindranath}, R.~Michael {Rich}, John
  {Ruan}, Jan {Rybizki}, Charli {Sakari}, Robyn~E. {Sanderson}, Ricardo
  {Schiavon}, Carlo {Schimd}, Aldo {Serenelli}, Arnaud {Siebert}, Malgorzata
  {Siudek}, Rodolfo {Smiljanic}, Daniel {Smith}, Jennifer {Sobeck}, Else
  {Starkenburg}, Dennis {Stello}, Gyula~M. {Szab{\'o}}, Robert {Szabo},
  Matthew~A. {Taylor}, Karun {Thanjavur}, Guillaume {Thomas}, Erik {Tollerud},
  Silvia {Toonen}, Pier-Emmanuel {Tremblay}, Laurence {Tresse}, Maria
  {Tsantaki}, Marica {Valentini}, Sophie {Van Eck}, Andrei {Variu}, Kim {Venn},
  Eva {Villaver}, Matthew~G. {Walker}, Yiping {Wang}, Yuting {Wang}, Michael~J.
  {Wilson}, Nicolas {Wright}, Siyi {Xu}, Mutlu {Yildiz}, Huawei {Zhang},
  Konstanze {Zwintz}, Borja {Anguiano}, Megan {Bedell}, William {Chaplin}, Remo
  {Collet}, Jean-Charles {Cuillandre}, Pierre-Alain {Duc}, Nicolas {Flagey},
  JJ~{Hermes}, Alexis {Hill}, Devika {Kamath}, Mary~Beth {Laychak}, Katarzyna
  {Ma{\l}ek}, Mark {Marley}, Andy {Sheinis}, Doug {Simons}, S{\'e}rgio~G.
  {Sousa}, Kei {Szeto}, Yuan-Sen {Ting}, Simona {Vegetti}, Lisa {Wells},
  Ferdinand {Babas}, Steve {Bauman}, Alessandro {Bosselli}, Pat {C{\^o}t{\'e}},
  Matthew {Colless}, Johan {Comparat}, Helene {Courtois}, David {Crampton},
  Scott {Croom}, Luke {Davies}, Richard {de Grijs}, Kelly {Denny}, Daniel
  {Devost}, Paola {di Matteo}, Simon {Driver}, Mirian {Fernandez-Lorenzo}, Raja
  {Guhathakurta}, Zhanwen {Han}, Clare {Higgs}, Vanessa {Hill}, Kevin {Ho},
  Andrew {Hopkins}, Mike {Hudson}, Rodrigo {Ibata}, Sidik {Isani}, Matt
  {Jarvis}, Andrew {Johnson}, Eric {Jullo}, Nick {Kaiser}, Jean-Paul {Kneib},
  Jun {Koda}, George {Koshy}, Shan {Mignot}, Rick {Murowinski}, Jeff {Newman},
  Adi {Nusser}, Anna {Pancoast}, Eric {Peng}, Celine {Peroux}, Christophe
  {Pichon}, Bianca {Poggianti}, Johan {Richard}, Derrick {Salmon}, Arnaud
  {Seibert}, Prajval {Shastri}, Dan {Smith}, Firoza {Sutaria}, Charling {Tao},
  Edwar {Taylor}, Brent {Tully}, Ludovic {van Waerbeke}, Tom {Vermeulen},
  Matthew {Walker}, Jon {Willis}, Chris {Willot}, and Kanoa {Withington}.
\newblock {The Detailed Science Case for the Maunakea Spectroscopic Explorer,
  2019 edition}.
\newblock {\em arXiv e-prints}, page arXiv:1904.04907, Apr 2019.

\bibitem{Thekkadath_21}
G.~S. Thekkadath, S.~Sempere-Llagostera, B.~A. Bell, et~al.
\newblock Single-shot discrimination of coherent states beyond the standard
  quantum limit.
\newblock {\em Optics Letters}, 46(11):2565--2568, 2021.

\bibitem{thorburn2021ge}
Fiona Thorburn, Xin Yi, Zo{\"e}~M Greener, Jaroslaw Kirdoda, Ross~W Millar,
  Laura~L Huddleston, Douglas~J Paul, and Gerald~S Buller.
\newblock Ge-on-si single-photon avalanche diode detectors for short-wave
  infrared wavelengths.
\newblock {\em Journal of Physics: Photonics}, 4(1):012001, 2021.

\bibitem{skipper2017}
Javier {Tiffenberg}, Miguel {Sofo-Haro}, Alex {Drlica-Wagner}, Rouven {Essig},
  Yann {Guardincerri}, Steve {Holland}, Tomer {Volansky}, and Tien-Tien {Yu}.
\newblock {Single-Electron and Single-Photon Sensitivity with a Silicon Skipper
  CCD}.
\newblock {\em \textit{PRL}}, 119(13):131802, Sep 2017.

\bibitem{Tiffenberg2017}
Javier Tiffenberg, Miguel Sofo-Haro, Alex Drlica-Wagner, Rouven Essig, Yann
  Guardincerri, Steve Holland, Tomer Volansky, and Tien-Tien Yu.
\newblock {Single-Electron and Single-Photon Sensitivity with a Silicon Skipper
  CCD}.
\newblock {\em Phys. Rev. Lett.}, 119:131802, Sep 2017.

\bibitem{Tingay:2020}
Steven {Tingay}.
\newblock {High-cadence optical transient searches using drift scan imaging I:
  Proof of concept with a pre-prototype system}.
\newblock {\em Publications of the Astronomical Society of Australia}, 37:e015,
  April 2020.

\bibitem{TISA2007113}
S.~Tisa, F.~Zappa, A.~Tosi, and S.~Cova.
\newblock Electronics for single photon avalanche diode arrays.
\newblock {\em Sensors and Actuators A: Physical}, 140(1):113--122, 2007.

\bibitem{tosi2012fully}
Alberto Tosi, Adriano Della~Frera, Andrea Bahgat~Shehata, and Carmelo
  Scarcella.
\newblock Fully programmable single-photon detection module for ingaas/inp
  single-photon avalanche diodes with clean and sub-nanosecond gating
  transitions.
\newblock {\em Review of Scientific Instruments}, 83(1):013104, 2012.

\bibitem{vachon2020measuring}
Fr{\'e}d{\'e}ric Vachon, Samuel Parent, Fr{\'e}d{\'e}ric Nolet, Henri Dautet,
  Jean-Francois Pratte, and Serge~A Charlebois.
\newblock Measuring count rates free from correlated noise in digital silicon
  photomultipliers.
\newblock {\em Measurement Science and Technology}, 2020.

\bibitem{Vachon20221-MScA}
Frédéric Vachon.
\newblock Conception de photodiodes à avalanche monophotonique sensibles aux
  photons ultraviolets pour les détecteurs de la physique des particules dans
  les gaz nobles liquéfiés.
\newblock Master's thesis, Université de Sherbrooke, Canada, May 2021.
\newblock {\textsc{url:}~\url{http://hdl.handle.net/11143/18350}}.

\bibitem{Vasiukov:2019hwn}
S.~Vasiukov, F.~Chiossi, C.~Braggio, G.~Carugno, F.~Moretti, E.~Bourret, and
  S.~Derenzo.
\newblock {GaAs as a bright cryogenic scintillator for the direct dark matter
  detection}.
\newblock 4 2019.

\bibitem{verghese2005geiger}
S~Verghese, DM~Cohen, EA~Dauler, JP~Donnelly, EK~Duerr, SH~Groves, PI~Hopman,
  KE~Jensen, Z-L Liau, LJ~Mahoney, et~al.
\newblock Geiger-mode avalanche photodiodes for photon-counting communications.
\newblock In {\em Digest of the LEOS Summer Topical Meetings, 2005.}, pages
  15--16. IEEE, 2005.

\bibitem{verma2021}
Varun~V Verma, Boris Korzh, Alexander~B Walter, Adriana~E Lita, Ryan~M Briggs,
  Marco Colangelo, Yao Zhai, Emma~E Wollman, Andrew~D Beyer, Jason~P Allmaras,
  Heli Vora, Di~Zhu, Ekkehart Schmidt, Alexander~G Kozorezov, Karl~K Berggren,
  Richard~P Mirin, Sae~Woo Nam, and Matthew~D Shaw.
\newblock Single-photon detection in the mid-infrared up to 10 $\mu$m
  wavelength using tungsten silicide superconducting nanowire detectors.
\newblock {\em APL Photonics}, 6:056101, 2021.

\bibitem{vines2019high}
Peter Vines, Kateryna Kuzmenko, Jaros{\l}aw Kirdoda, Derek Dumas, Muhammad~M
  Mirza, Ross~W Millar, Douglas~J Paul, and Gerald~S Buller.
\newblock High performance planar germanium-on-silicon single-photon avalanche
  diode detectors.
\newblock {\em Nature communications}, 10(1):1--9, 2019.

\bibitem{2020PASP..132l5005W}
Alexander~B Walter, Neelay Fruitwala, Sarah Steiger, John I~III Bailey,
  Nicholas Zobrist, Noah Swimmer, Isabel Lipartito, Jennifer~Pearl Smith,
  Seth~R Meeker, Clint Bockstiegel, Gr{\'e}goire Coiffard, Rupert Dodkins, Paul
  Szypryt, Kristina~K Davis, Miguel Daal, Bruce Bumble, Giulia Collura, Olivier
  Guyon, Julien Lozi, S{\'e}bastien Vievard, Nemanja Jovanovic, Frantz
  Martinache, Thayne Currie, and Benjamin~A Mazin.
\newblock {The MKID Exoplanet Camera for Subaru SCExAO}.
\newblock {\em Publications of the Astronomical Society of the Pacific},
  132(1):125005, December 2020.

\bibitem{Wang_22}
G.~Wang, C.~L. Chang, M.~Lisovenko, et~al.
\newblock Light dark matter detection with hydrogen-rich crystals and low-{Tc}
  {TES} detectors.
\newblock arXiv:2201.04219, 2022.

\bibitem{warburton2013ge}
Ryan~E Warburton, Giuseppe Intermite, Maksym Myronov, Phil Allred, David~R
  Leadley, Kevin Gallacher, Douglas~J Paul, Neil~J Pilgrim, Leon~JM Lever,
  Zoran Ikonic, et~al.
\newblock Ge-on-si single-photon avalanche diode detectors: design, modeling,
  fabrication, and characterization at wavelengths 1310 and 1550 nm.
\newblock {\em IEEE Transactions on Electron Devices}, 60(11):3807--3813, 2013.

\bibitem{Weii_08}
D.~Wei, J.~Olaya, B.~S. Karasik, et~al.
\newblock Ultrasensitive hot-electron nanobolometers for terahertz
  astrophysics.
\newblock {\em Nature nanotechnology}, 3(8):496--500, 2008.

\bibitem{Weiss2017}
David~S. Weiss and Martin Abkowitz.
\newblock {\em Organic Photoconductors}, pages 1--1.
\newblock Springer International Publishing, Cham, 2017.

\bibitem{Radeka1974}
W.J. Willis and V.~Radeka.
\newblock Liquid-argon ionization chambers as total-absorption detectors.
\newblock {\em Nucl. Instrum. Meth.}, 120(2):221 -- 236, 1974.

\bibitem{Wollman:2019}
Emma~E. Wollman, Varun~B. Verma, Adriana~E. Lita, William~H. Farr, Matthew~D.
  Shaw, Richard~P. Mirin, and Sae~Woo Nam.
\newblock Kilopixel array of superconducting nanowire single-photon detectors.
\newblock {\em Opt. Express}, 27(24):35279--35289, Nov 2019.

\bibitem{wollman2019kilopixel}
Emma~E Wollman, Varun~B Verma, Adriana~E Lita, William~H Farr, Matthew~D Shaw,
  Richard~P Mirin, and Sae~Woo Nam.
\newblock Kilopixel array of superconducting nanowire single-photon detectors.
\newblock {\em Optics express}, 27(24):35279--35289, 2019.

\bibitem{Zabrodskii:2015pda}
V.~Zabrodskii et~al.
\newblock {SiPM prototype for direct VUV registration}.
\newblock {\em Nucl. Instrum. Meth.}, A787:348--352, 2015.

\bibitem{zappa1994nanosecond}
Franco Zappa, A~Lacaita, Sergio Cova, and P~Webb.
\newblock Nanosecond single-photon timing with ingaas/inp photodiodes.
\newblock {\em Optics letters}, 19(11):846--848, 1994.

\bibitem{zappa1996temperature}
Franco Zappa, P~Lovati, and A~Lacaita.
\newblock Temperature dependence of electron and hole ionization coefficients
  in inp.
\newblock In {\em Proceedings of 8th International Conference on Indium
  Phosphide and Related Materials}, pages 628--631. IEEE, 1996.

\bibitem{1997-Zappa_SPAD}
P.~Zappa, M.~Ghioni, S.~Cova, L.~Varisco, B.~Sinnis, A.~Morrison, and
  A.~Mathewson.
\newblock Integrated array of avalanche photodiodes for single-photon counting.
\newblock In {\em 27th european solid-state device research conference}, pages
  600--603, {Stuttgart, Germany}, 1997.

\bibitem{doi:10.1118/1.2903425}
Bo~Zhao and Wei Zhao.
\newblock Imaging performance of an amorphous selenium digital mammography
  detector in a breast tomosynthesis system.
\newblock {\em Medical Physics}, 35(5):1978--1987, 2008.

\bibitem{2019ApPhL.115d2601Z}
Nicholas Zobrist, Byeong~Ho Eom, Peter Day, Benjamin~A Mazin, Seth~R Meeker,
  Bruce Bumble, Henry~G Leduc, Gr{\'e}goire Coiffard, Paul Szypryt, Neelay
  Fruitwala, Isabel Lipartito, and Clint Bockstiegel.
\newblock {Wide-band parametric amplifier readout and resolution of optical
  microwave kinetic inductance detectors}.
\newblock {\em Applied Physics Letters}, 115(4):042601, July 2019.


\bibitem{PhotonCountingWP}
Jonathan Asaadi et al.
\newblock Photon counting from the vacuum ultraviolet to the short wavelength infrared using semiconductor and superconducting technologies.
\newblock {\em arXiv preprint arXiv:2203.12542}, 2022.

\bibitem{APDHep}
Francesco Gramuglia et al.
\newblock Sub-10 ps Minimum Ionizing Particle Detection with Geiger-Mode APDs.
\newblock {\em arXiv preprint arXiv:2111.09998 }, 2021.


==> Instrumentation/bibliography.tex <==

\bibitem{I4-Scoresby}
J. Scoresby, ``Journals'', 1820.

\bibitem{I-Beale}
A. Beale, ``Surgical Writings'', 1839.



==> tcilcomm.tex <==
% Macros used for TCI styles released with Scientific Word 1.1.
%Copyright (C) 1992-93 TCI Software Research, Inc.
\typeout{TCILCOMM Macros for TCI styles <08 Apr 93>.}
%
% Revisions:
% 08 Apr 93 - GP change line length to under 80 characters
% 30 Mar 92 - AO added \setmoremathsizes and hooks to, e.g. \@xpt,
%             for support of bold Greek
%
%%ltg added this to try to get 12pt to come through
%\DeclareOption{12pt}{\renewcommand\@ptsize{2}}
%%end ltg

\def\@ptoptions{%
 \let\@elt\relax\@for\@tempa:=\@optionlist\do{%
  \expandafter\let\expandafter\@tempb\csname ds@\@tempa\endcsname
  \expandafter\let\expandafter\@tempc\csname ds@11pt\endcsname
  \ifx\@tempb\@tempc\else
   \expandafter\let\expandafter\@tempc\csname ds@12pt\endcsname
   \ifx\@tempb\@tempc\else\let\@tempb\relax\fi
   \fi
  \@tempb
  }%
 }%
%
% read in style file, but only process the pt size options
%
\def\@ptoptinput#1{%
 \let\@save@optionlist\@optionlist
 \let\@save@options\@options
 \let\@options\@ptoptions
 %
 \input #1
 %
 \let\@optionlist\@save@optionlist
 \let\@options\@save@options
 }%
%
% the <21 Feb 92> version of letter.sty requires:
\ifx\undefined\reset@font
 \def\reset@font{}%
 \fi
%
% Change LaTeX
%
% Add command to append tokens
\newtoks\@temptokenb
\long\def\appdef#1#2{%
 \ifx#1\undefined\let#1\@empty\fi
 \@temptokena\expandafter{#1}\@temptokenb{#2}%
 \edef#1{\the\@temptokena\the\@temptokenb}%
 }%
\long\def\prepdef#1#2{%
 \ifx#1\undefined\let#1\@empty\fi
 \@temptokena\expandafter{#1}\@temptokenb{#2}%
 \edef#1{\the\@temptokenb\the\@temptokena}%
 }%
% Discard contents of \box\@cclv at beginning of document
\appdef\document{{\output{\setbox\z@\box\@cclv}\endgraf\null\eject}}%
% Fix mark register expansion
\def\leftmark{\expandafter\@leftmark\botmark{}{}{}\@nil}%
\def\rightmark{\expandafter\@rightmark\firstmark{}{}{}\@nil}%
\def\@leftmark#1#2#3\@nil{#1}%
\def\@rightmark#1#2#3\@nil{#2}%
%
%\show\raggedright
\newskip\raggedglue
\raggedglue\z@ plus20\p@ minus\z@
\def\raggedright{%
 \let\\=\@centercr\@rightskip\raggedglue\rightskip
 \@rightskip\leftskip\z@\parindent\z@
 }%
%
\def\@centercr{%
 \ifhmode\unskip\else\@badcrerr\fi\@@par
 \@ifstar{\penalty\@M\@xcentercr}{\@xcentercr}%
 }%
%
\def\traceoutput{\tracingoutput2\showboxbreadth\maxdimen
 \showboxdepth\maxdimen}%
%
\newcount\@hour\newcount\@minute\chardef\@x10\chardef\@xv60
\def\@time{%
  \@minute\time\@hour\@minute\divide\@hour\@xv
  \ifnum\@hour<\@x 0\fi\the\@hour:%
  \multiply\@hour\@xv\advance\@minute-\@hour
  \ifnum\@minute<\@x 0\fi\the\@minute
  }%
%
% change \@array to allow \par to mean something within its scope
%
\def\@array [#1]#2{%
 \setbox\@arstrutbox\hbox{\vrule height\arraystretch\ht
  \strutbox depth\arraystretch\dp\strutbox width\z@}%
 \@mkpream{#2}%
 \edef\@preamble{\halign\noexpand\@halignto\bgroup\tabskip
  \z@\@arstrut\@preamble\tabskip\z@\cr}%
 \let\@startpbox\@@startpbox\let\@endpbox\@@endpbox
 \if#1t\vtop\else\if#1b\vbox\else\vcenter\fi\fi
 \bgroup
  %\let\par\relax
  \let\@sharp##
  \let\protect\relax
  \lineskip\z@\baselineskip\z@
  \@preamble
 }%
%
% Expands to hex digit corresponding to the value of the argument
%
\def\hexnumber@#1{\ifnum#1<10 \number#1\else
 \ifnum#1=10 A\else\ifnum#1=11 B\else\ifnum#1=12 C\else
 \ifnum#1=13 D\else\ifnum#1=14 E\else\ifnum#1=15 F\fi\fi\fi\fi\fi\fi\fi}%
%
% define command to set more math sizes.
% Styles like Greekbf will hook in here.
%
\def\setmoremathsizes#1#2#3{}%
%
% define size switch addenda
%  Note: these choices agree with those in lfonts.tex, even if incorrect.
%
\prepdef\@vpt{\setmoremathsizes{fiv}{fiv}{fiv}}%
\prepdef\@vipt{\setmoremathsizes{six}{six}{six}}%
\prepdef\@viipt{\setmoremathsizes{sev}{fiv}{fiv}}%
\prepdef\@viiipt{\setmoremathsizes{egt}{six}{fiv}}%
\prepdef\@ixpt{\setmoremathsizes{nin}{six}{fiv}}%
\prepdef\@xpt{\setmoremathsizes{ten}{sev}{fiv}}%
\prepdef\@xipt{\setmoremathsizes{elv}{egt}{six}}%
\prepdef\@xiipt{\setmoremathsizes{twl}{egt}{six}}%
\prepdef\@xivpt{\setmoremathsizes{frtn}{ten}{sev}}%
\prepdef\@xviipt{\setmoremathsizes{svtn}{twl}{ten}}%
\prepdef\@xxpt{\setmoremathsizes{twty}{frtn}{twl}}%
\prepdef\@xxvpt{\setmoremathsizes{twty}{twty}{svtn}}%
%
% The \newfield command defines (like \newenvironment) a user syntax:
%
%   \newfield{foo}
%
% lets you write
%
%   \begin{foo}...\end{foo}
%
% but differs from \newenvironment in that TeX parses the entire content
% of the field and stores it in a macro \the@foo, and then executes \@do@foo.
%
% This means that the content of the field is actually more like an argument
% than the content of an environment. So \verb will not necessarily work
% within a field, and neither will \index. Caveat emptor.
%
% The default procedure for a field is to process its argument within a
% group.  If you want a field to simply store its data away, define its
% procedure to be synonymous with \@empty, as illustrated below.
%
\long\def\@readenvir#1#2\end{%
 \appdef\envirsofar{#2}%
 \@ifnextchar\bgroup{\@checkenvir{#1}}{\@envirenderr}%
 }%
%
\def\@envirenderr{%
 \@latexerr{\string\end\space not followed by environment name}\@eha
 }%
%
\def\@checkenvir#1#2{%
 \def\@tempa{#1}\def\@tempb{#2}%
 \ifx\@tempa\@tempb
  \ifx\envirsofar\@blankspace\let\envirsofar\@empty\fi
  \expandafter\let\csname the@#1\endcsname\envirsofar
  \def\@tempa{\csname @do@#1\endcsname}%
  \else
  \appdef\envirsofar{\end{#2}}%
  \def\@tempa{\@readenvir{#1}}%
  \fi
 \@tempa
 }%
%
\def\newfield#1#2{%
 \expandafter\@ifdefinable\csname#1\endcsname{%
  \expandafter\def\csname#1\endcsname{%
   \endgroup\let\envirsofar\@empty\@readenvir{#1}%
   }%
  \expandafter\let\csname the@#1\endcsname\@empty
  \expandafter\ifx\csname @do@#1\endcsname\relax
   \expandafter\def\csname @do@#1\endcsname{{\csname the@#1\endcsname}}%
   \fi
  }%
 }%
%
\def\@blankspace{ }% SciWord's nil field
%
\def\letparBL{\def\par{\\}}%
\def\letparSP{\def\par{\ }}%
\def\letparQD{\def\par{\quad}}%
\def\letparSL{\def\par{\hbox to1em{\hfil/\hfil}}}%
%
% When \par is processed in the page head, gobble up the rest of the
% argument.
\def\@gobblepar#1\@empty{}%
%
% Physical page size after trim
\newdimen\trimwidth
\newdimen\trimheight
\newdimen\botmargin
\newdimen\marginpartotal
%
\def\adjustpagemargin{% adjust \oddsidemargin by \marginpartotal
 \marginpartotal\marginparwidth\advance\marginpartotal\marginparsep
 \advance\oddsidemargin\marginpartotal
 }%
%
\def\settextheight{% calculate textheight constrained by:
 \textheight\trimheight
 \advance\textheight-\topmargin
 \advance\textheight-\headheight
 \advance\textheight-\headsep
 \advance\textheight-\footskip
 \advance\textheight-\botmargin
 }%
%
\def\vcenterpagemargin{% calculate \topmargin constrained by:
 \topmargin\trimheight
 \advance\topmargin-\textheight
 \advance\topmargin-\headheight
 \advance\topmargin-\headsep
 \advance\topmargin-\footskip
 \divide\topmargin\tw@\botmargin\topmargin
 }%
%
\def\centerpagemargin{% calculate \oddsidemargin constrained by:
 \oddsidemargin\trimwidth
 \advance\oddsidemargin-\textwidth
 \advance\oddsidemargin-\marginparwidth
 \advance\oddsidemargin-\marginparsep
 \divide\oddsidemargin\tw@
 \evensidemargin\oddsidemargin
 \adjustpagemargin
 }%
%
\def\leftpagemargin{% calculate \oddsidemargin constrained by:
 \oddsidemargin\trimwidth
 \advance\oddsidemargin-\textwidth
 \advance\oddsidemargin-\marginparwidth
 \advance\oddsidemargin-\marginparsep
 \advance\oddsidemargin-\evensidemargin
 \adjustpagemargin
 }%

